Dense Passage Retrieval in Conversational Search

Information retrieval systems have traditionally relied on exact term match methods such as BM25 for first-stage retrieval. However, recent advancements in neural network-based techniques have introduced a new method called dense retrieval. This approach uses a dual-encoder to create contextual embeddings that can be indexed and clustered efficiently at run-time, resulting in improved retrieval performance in Open-domain Question Answering systems. In this paper, we apply the dense retrieval technique to conversational search by conducting experiments on the CAsT benchmark dataset. We also propose an end-to-end conversational search system called GPT2QR+DPR, which incorporates various query reformulation strategies to improve retrieval accuracy. Our findings indicate that dense retrieval outperforms BM25 even without extensive fine-tuning. Our work contributes to the growing body of research on neural-based retrieval methods in conversational search, and highlights the potential of dense retrieval in improving retrieval accuracy in conversational search systems.

==> ANCE/Abs.tex <==
\vspace{-0.3cm}\begin{abstract}\vspace{-0.1cm}
Conducting text retrieval in a dense representation space has many intriguing advantages. Yet the end-to-end learned dense retrieval (DR) often underperforms word-based sparse retrieval. In this paper, we first theoretically show the learning bottleneck of dense retrieval is due to the domination of uninformative negatives sampled locally in batch, which yield diminishing gradient norms, large stochastic gradient variances, and slow learning convergence. We then propose Approximate nearest neighbor Negative Contrastive Learning (ANCE), a learning mechanism that selects hard training negatives globally from the entire corpus, using an asynchronously updated ANN index. Our experiments demonstrate the effectiveness of ANCE on web search, question answering, and in a commercial search environment, showing ANCE dot-product retrieval nearly matches the accuracy of BERT-based cascade IR pipeline, while being 100x more efficient. \vspace{-0.1cm}
% We also empirically validate our theory that ANCE better approximates the oracle gradient-norm based importance sampling.
% , thus improves the convergence.
% of stochastic training.
\end{abstract}


==> ANCE/Arxiv/Intro.tex <==
\section{Introduction}

\cx{
Our main contribution:
\begin{enumerate}
    \item A new ANN NCE training framework that provides more effective and aligned training for dense retrieval, fixed the mismatch in negatives in learning and inference
    \item the first to outperform sparse retrieval in real IR document tasks with pure dense retrieval and outperforms all previous dense retrieval/representation based retrieval methods by large 
    \item thorough analyses illustrating the ANN-NCE learning process and its influence. 
    % \ja{Can we allude to SOTA results on representation based information retrieval of relevant results ? done, #2}
\end{enumerate}
}

% \cx{Outlines. Each bracket is }



% \cx{where we are in language AI: beyond human in later stage, rule-based 40 years old BM25 in first stage}
Many NLP-focused systems rely on text retrieval to find relevant information as input for later inference stages. For example,
search ranking~\cite{nogueira2019passage}, answer span extraction~\cite{chen2017reading}, multi-hop reasoning~\cite{yang2018hotpotqa, thorne2018fact}, grounded conversation response generation~\cite{zhou2018dataset} all assume extracting from the broad set of all items a set of filtered ``mostly relevant'' candidates on which a more computationally expensive ranking, extraction, classification, or generation step is run. All these ``later stage modules'' have enjoyed the revolutionary advantages from distributed, pretrained, and end-to-end deep learning models, and reached ``beyond human performances'' in many public benchmarks~\cite{rajpurkar2016squad, wang2018glue}. In contrast, the first stage retrieval part, which provides the basic information for the later components in these AI systems, is often still based on the sparse, bag-of-words, representations and exact matches within~\cite{chen2017reading, zhaotransxh2020, yang2018hotpotqa, nogueira2019passage}.
BM25~\cite{bm25}, unsupervised sparse retrieval using hand-crafted rules, is still a strong baseline and sometimes even the state-of-the-art, 40 years after its invention~\cite{zamani2018neural, karpukhin2020dense, luan2020sparsedense, lee2019latent}.



The limited capability of the sparse first retrieval enforces a potential upper bound of modern language AI systems.
The intrinsic challenge of sparse retrieval, i.e. vocabulary mismatch and language varieties~\cite{croft2010search}, brings in noisy and missed information in the first stage, which is challenging, sometimes impossible \ao{should this statement be stronger? there should be many queries where context isn't captured by keyword matching, resulting in BM25 to miss the document at L1 which cannot be recovered from in later stages}, \ja{I would add that in a multi-step search process, the first step fundamentally limits the second step, which is what Arnold is also alluding to \cx{Yes. Now it is doing the same purpose but I should spend more space on the challenge part.}}for the later deep neural models to recover~\cite{yang2018hotpotqa, craswell2020overview}. 




% \cx{The importance of dense retrieval:
% \begin{enumerate}
%     \item resolve the bottleneck in e2e information system
%     \item unleash the full potential of neural methods in many downstream applications
%     \item unified and easier to maintain infrastructure
%     \item Also Pretrained LM and ANN inference are getting ready
% \end{enumerate}
% }
% \cx{The observations and challenges in recent progress:
% \begin{enumerate}
%     \item good for short passage but not as good on longer passage
%     \item reranking is promising but not yet fully e2e retrieval, many times have to combine with sparse model
%     \item even some permissive analyses that the capacity of encoding has to be very high for documents
% \end{enumerate}
% }

Dense retrieval, which learns retrieval texts using the learned distributed embeddings, is a promising potential direction to overcome the sparse retrieval bottleneck~\cite{lee2019latent, chang2020pre, luan2020sparsedense, gao2020complementing, ma2020zero, dhingra2020differentiable, karpukhin2020dense}: The representation space is end-to-end learned,  tailored for the task, leverages the strength of language model pretraining, while also being sufficiently efficient thanks to the recent progress in Approximate Nearest Neighbor (ANN) search~\cite{johnson2019billion}. \ja{minor point: I wonder if the statement above where we say that BM25 is state of the art and that dense retrieval already has many citations (and hence are proven better than BM25) could conflict ? \cx{citations is not equal to better, many dense retrieval paper show they are not as strong on longer texts.}}

One would expect learned dense representation to revolutionize the first stage retrieval, as they have in many other language tasks. However, this is not necessarily the case in text retrieval: Recent studies often found that dense retrieval with BERT sometimes under performs or is merely on-par with BM25, especially on long texts~\cite{luan2020sparsedense, lee2019latent}, raising concerns whether it is sustainable \ja{maybe a better way than sustainable is a more performant solution or has better ROI than BM25. \cx{Yes, it is a little subtle, we don't want to attack the ROI of our dense retrieval but need to say it was hard before this work.}} for document retrieval~\cite{luan2020sparsedense}, and the effectiveness of dense retrieval is mainly when combined with spare retrieval~\cite{gao2020complementing, ma2020zero}---as an add-on to BM25, but not yet a next-gen retrieval.





% \cx{Our solution:
% \begin{enumerate}
%     \item We identified the main bottleneck is actually in the training phrase, the mismatch between negatives seem in training and ANN inference
%     \item Developed a new training mechanism in the NCE framework, but instead of in-batch sampling, we directly do that in ANN, which is exact how the dense retrieval model is to be used
% \end{enumerate}
% }

In this paper we identify the main reason of such underwhelming performance of dense retrieval, especially on longer texts, is the learning part. Specifically, the mismatches of negatives sampled for training and the actually negatives in retrieval. 
% \ja{Previous sentence and next sentence are both technically strong and convey vital aspect of understanding; consider : Too many commas, suggest breaking down the long sentence for better readability}
In training, the negatives is either randomly sampled, selected in nearby batches, or from the sparse retrieval, following standard learning to rank settings~\cite{liu2009learning}. However, when testing, the trained model needs to retrieve the relevant documents in the entire corpus, e.g., via ANN, which is drastically different  from the negatives in sparse retrieval nor the random sampled negatives can provide the minutiae required for ranking among the top retrievals ($\mathsection$~\ref{sec:ancenegatives}). 


% \cx{More details of ANCE:
% \begin{enumerate}
%     \item We build ANN index with the doc representations
%     \item directly pick negatives from the ANN for each q and d+ label
%     \item refresh ANN after certain steps, as asynchronous updates
%     \item until converges in validation
% \end{enumerate}
% }

We eliminate this mismatch with Approximate nearest neighbor Noise Contrastive Estimation (ANCE), which follows the principle of NCE~\cite{gutmann2010noise, mnih2013learning, oord2018representation}, and selects stronger, \textit{more realistic}, negatives from an ANN index in learning. The ANN index includes the encodings of the documents/passages, from the same representation model being learned for the dense retrieval, and is parallelly updated and asynchronously refreshed as the optimization goes on. The negatives are sampled from this ANN index using the same retrieval function (dot product, e.g.), the same representation model (though delayed due to the asynchronous index update). Thus the training negatives are much more aligned with the actual negatives dense retrieval models would encounter in real world. \ja{Could we say that this is an "effective hard negative sampling problem" addressed through elegant use of lower ranked documents ? I personally found the analogy with hard negative which is a well known ML concept quite apt but not sure if that resonates with research community \cx{It is doing this? I will make the point more crisp. Note that NCE, InfoNCE is doing strong negative selection, we are just doing it better and more fundemental.}}





% \cx{Our contribution as shown in experiments:
% \begin{enumerate}
%     \item The first to outperform all sparse retrieval, BM25 and beyond, as well as feature-based LeToR on TREC DL Doc task, a realistic, large scale, document retrieval task from Bing queries and documents.  
%     \item stronger than other training mechanisms: NCE, in batch, BM25+NCE, etc. (hopefully also momentum).
%     \item All with vanilla BERT-Siamese,  works for both doc ranking and passage ranking, with simple max-pooling or longformer on doc side.
% \end{enumerate}
% }

In TREC Deep Learning Track's large scale document and passage ranking benchmarks~\cite{craswell2020overview}, ANCE significantly boost the retrieval accuracy of dense retrieval. With ANCE training, the vanilla BERT-Siamese dual encoder, the same architecture used in several parallel research~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}, significantly outperforms all dense retrieval baselines, many with same architecture but different training scheme, and sparse retrieval methods, not only BM25, but also its stronger variations developed in core ad hoc retrieval.  
ANCE in fact empowers vanilla BERT-Siamese to outperform many two-stage retrieval-and-reranking systems~\cite{liu2009learning, www2017duet}, solely via one dense retrieval step with dot-product in the representation space. This overwhelming effectiveness
% \ja{overwhelming effectiveness} 
is the first we have seen in dense document retrieval, and our analyses provide further insights and illustrate how ANCE effectively trains the encoders for more robust and accurate dense retrieval.



% \cx{Our insights:
% \begin{enumerate}
%     \item the main gain is from our ANCE training, without it, there is a clear gap in reranking and retrieval, and our analyses show how the gap of different negatives are resolved during the ANCE training.
%     \item More details in how/when to refresh index, the LR scheduling, warm up, and negative sampling, to shine lights of representation learning in other related tasks
%     \item case studies to show the different behavior of dense retrieval and sparse retrieval 
% \end{enumerate}
% }

==> ANCE/Arxiv/doc_res.tex <==
\lx{this is placeholder template until numbers are fully replaced}
\begin{table*}[ht]
    \centering
    \small
    % \begin{adjustbox}{width=0.95\textwidth,center}
    \begin{tabular}{l|cc|cc|cc} \hline \hline
    & \multicolumn{2}{c|}{\textbf{MARCO Dev}} 
    & \multicolumn{2}{c|}{\textbf{TREC Rerank}} 
    & \multicolumn{2}{c}{\textbf{TREC Retrieval}}
    \\ \hline  
    % \textbf{Method}     
    % &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c|}{\textbf{Recall@5}}
    %   &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c}{\textbf{Recall@5}}
    % \\ \hline
           \textbf{Method}     
    &  \textbf{MRR@10} &  \textbf{Recall@1k}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
    \\ \hline
{BM25} 
& 0.31 & ~ & N/A & N/A & 0.52 & 2\% \\
{Best DeepCT}~\cite{dai2019context} & \\
{TREC Best Retrieval}  & \\
{TREC Best Trad} & 
\\ \hline
{BERT Ranker}~\cite{nogueira2019passage}  % from literature 
& -- & -- & 0.64 & ~  & -- & -- 
\\\hline

%
%{\textbf{*Document Warmup}} \cx{move this to appendix \lx{ablation study or appendix?} } & ~ & 0.35 & ~ & ~ & ~ & ~ & ~  \\ %/webdata-nfs/yeli1/msmarco_doc_5M_30k/rdot_nll_128_bm25/checkpoint-84000/
%{w/ ANCE - 512} & ~ & 0.56 & ~ & ~ & ~ & ~ & ~   \\
%\hline

{\textbf{Dense Retrieval}}   \\
BM25 $\rightarrow$ Random Neg \\
%checkpoint_path = "/mnt/azureblob/lexion/doc_checkpoint/"
%checkpoint = 0

{NCE Neg}~\cite{gutmann2010noise} \\

{BM25 + Random}~\cite{luan2020sparsedense, karpukhin2020dense} 
& ~ & ~ & 0.630 & 2.5\% & 0.539 & 26\%   \\
% checkpoint_path = "/webdata-nfs/lexion/msmarco_doc_5M_30k/final_IB_BM25_measure/"
%checkpoint = 0

{w. ANCE (512)} & ~ & ~ & 0.641 & 3\% & 0.615 & 13\%    \\ 
%checkpoint_path = "/mnt/azureblob/lexion/doc_checkpoint/"
%checkpoint = 210000

{w. ANCE (2048)} & ~ & ~ & ~ & ~ & 0.625 & ~ %checkpoint_path = "/webdata-nfs/yeli1/msmarco_doc_5M_30k/rdot_null_2048_lr1e-5/"
%checkpoint = 139000

\\

\hline \hline
    \end{tabular}
     \caption{TREC DL Track 2019 Document 
    \label{tab:doc_overal}}
%   \end{adjustbox}
\end{table*}



==> ANCE/Arxiv/efficiency.tex <==
\begin{sbsfigure*}
\centering
\small
\begin{tabular}{l|c|c} \hline \hline
\textbf{Operation} & \textbf{Offline}  & \textbf{Online } \\ \hline
    {\textbf{Sparse \& Cascade IR }} & \\
    {BM25 Retrieval} & & TODO  \\
    {Bert Rerank} & & 1.15s  \\
    {BM25 $\rightarrow$ Bert Reranker}  & & BM25+1.15s \\ \hline
    
    {\textbf{Dense IR }} & \\
    {ANCE Doc Encoding} & 10h per 8m doc &  \\
    {ANCE Query Encoding} & & 2.6ms \\
    \hline
    {\textbf{ANN Lookup}} &   \\
    {10 Query Batch} & 0.3s \\
    {100 Query Batch} &  92ms \\
    {1k Query Batch} & 9ms
    \\\hline
    {\textbf{End-to-End}}  & \\
   
    {ANCE Embedding} & 11.6ms \\
    \hline\hline
    {\textbf{ANCE Training}} &  \\
    {ANCE Corpus Inference} & 10h \\
    {ANN Index Build} & 10s \\
    {ANCE Training Set Build } & 5m  \\
    {Encoder Backprop} & 19ms \\
    \hline
    \end{tabular}
\end{sbsfigure*}



==> ANCE/Arxiv/efficiency_training_tbl.tex <==
\lx{TODO: place holder for runtime efficiencies}

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|c} \hline \hline
      & \multicolumn{1}{c}{\textbf{Time}} 
    \\  \hline

{\textbf{ANCE Training}} &  \\
{ANCE Corpus Inference} & 10h \\
{ANN Index Build} & 10s \\
{ANCE Training Set Build } & 5m  \\
{Encoder Backprop (1query, 1 positive, 1 negative)} & 19ms
\\\hline


\hline \hline
    \end{tabular}
     \caption{Measurement performed on single 32GB V100 GPU, XXX CPU, 660GB Memory 
     ~\label{tab:train_efficiency}}
\end{table*}



==> ANCE/Arxiv/eval.tex <==
\section{Evaluation Results}
\input{Tables/doc_pass_combined}
\input{Tables/openqa}


This section presents evaluation results on ANCE effectiveness and efficiency, and analyses on the Asynchronous learning. More evaluations and case studies can be found in Appendix.

\subsection{Effectiveness of ANCE Dense Retrieval}

The overall ranking accuracy in TREC Deep Learning Track benchmarks is presented in Table~\ref{tab:overall}. The main evaluation of DR methods is on their Retrieval accuracy from the ANN index; we also include their accuracy when Reranks top 100 documents retrieved by BM25.
% We separate the retrieval baselines from the reranking one for better comparisons. 
% For all DR methods, we mainly focus on their accuracy in the dense retrieval setting, using dot product in the ANN index, while we also include their results when used as a reranker on top of BM25 first stage retrieval.

ANCE empowers the DR model significantly outperforms all sparse retrieval baselines in all evaluation metrics. 
Not only it lead to 20\%+ NDCG gains over BM25 in all retrieval evaluations both passage retrieval and document retrieval, it also significantly outperforms the well-tuned best TREC traditional retrieval and best feature-based reranking models by large margins. Different from recent concerns on whether a single dense vector is sufficient for document DR, both ANCE (FirstP) and ANCE (MaxP) significantly advance the stage-of-the-art in document retrieval, without using any sparse information during retrieval---compared to DeepCT, which uses BERT to optimize sparse retrieval~\cite{dai2019transformer}, ANCE trained DR models enjoy 10\% better NDCG without replying on any BOW information. Similar advantages are also reflected in the MARCO Passage Retrieval in both MRR and recall.




Among all the learning mechanisms recently developed to train DR models, the best mechanism besides ANCE is to use a combination of BM25 negatives and random negatives: the sparse retrieval leads to a natural ``dictionary'' to select negatives for langauge related tasks, as discussed in multiple parallel work~\cite{gao2020complementing, ma2020zero, luan2020sparsedense, karpukhin2020dense, he2019momentum}. Yet there is almost always a 10\% gap from other methods to ANCE training---though all these approaches use the exact same DR model, the vanilla BERT-Siamese network. To the best of our knowledge, ANCE is the only method that enables dense retrieval to robustly outperform the best tuned sparse method in document ranking tasks. Section~\ref{sec:efficiency} further studies how the better negatives in the asynchronous learning of ANCE lead to this overwhelming effectiveness.

We found it promising to see BERT-Siamese, with ANCE training, nearly matches or even outperforms the interaction-based BERT reranker. This contradicts previous observations in Neu-IR, that the matches between query terms and document terms in the discrete BOW space is a necessity for neural ranking models~\cite{xiong2017knrm, guo2016deep, qiao2019understanding}. Many of the previous negative results upon BERT dual-encoders in Neu-IR perhaps are due to the challenges in model training rather than the network architecture. The same representation based BERT even outperforms the interaction-based BERT in document ranking. Not only that, in document retrieval, the bottleneck preventing end-to-end learned systems in many language AI systems, the ANCE trained DR model is less than 3\% away from the complex and state-of-the-art cascade IR pipeline which employs spare retrieval and then BERT Reranker, while only using the perhaps simplest dot product function in retrieval. 
In Section~\ref{sec:efficiency}, we discuss how this leads to very promising ``return of investiments'' (ROI) in computing resources.

\input{Tables/efficiency}
\subsection{Efficiency of ANCE Retrieval and Learning}
\label{sec:efficiency}

Table~\ref{tab.efficiency} measures the efficiency of different operations used in sparse retrieval, cascade IR pipeline, ANN dense retrieval, and ANCE's Asynchronous learning process.
Note that these numbers are measured in our commodity CPU/GPU server, with the open source toolkits we used. They may vary with different hardware, different implementation, paralleling, and distillation---though we expect the trend will remain mostly unchanged.

With batching, dot prod with FAISS ANN on CPU is sufficiently efficient. In high throughput environment such as commercial search, with sufficient query traffic to batch, fetching the document in the ANN index with dot prod is as efficient as from BM25's inverted index. 
Compared to Cascade IR, DR with BERT-Siamese enjoys much greater efficiency, especially online. The document encoding is calculated offline, i.e. in the crawling phrase of web search, and stored in the index; only the query encoding is required online, which requires less than 3ms and can be easily cached. In comparison, ranking with interaction-based BERT requires conducting inference on all the top K retrieved documents from BM25, which in theory is at least $O(K \times \frac{|q|+|d|}{|q|})$ times more expensive than DR ($|q|$ and $|d|$ refers to their lengths). In our experiment it requires more than one second per query, in comparison to DR's 11ms in high throughput environment, where efficiency matters the most. 

The cost Cascade IR with BERT ranker is often prohibitive latency wise or computing resource wise in many real systems, thus requires various approaches to speed up, e.g., to compute part of the transformer representations offline and cache them~\cite{}, to only use a few lower transformer layers~\cite{}, or to do task-specific distillation~\cite{}, all enforce certain efficiency-effectiveness trade-off. In comparison, our DR is 100 times more efficient, with 97\% accuracy, solely using a simple dot prod operation in the first stage retrieval.
This leads to remarkable ROI with reduced computing resource, energy consumption, and overhead on maintaining complicated pipelines.

In the ANCE Training phrase, Table~\ref{tab.efficiency} shows that the main bottleneck is not in the ANN part. Building the ANN Index or constructing the negative for the entire training query only takes seconds or minutes, which is perfectly fine in synchronous setting. However, the main bottleneck is to update the encodings of the document in the index, which requires a BERT inference of all the 8 Million training documents. This makes some type of asynchronous training almost inevitable in stochastic learning: the representation model is being updated per training batch, e.g., $n$ documents, $n<128$ per GPU. To keep the representations used in negative construction synchronous, one needs to refresh the encoding of all potential negatives, e.g. $m$ document, $m>1,000,000$, which is a $\frac{m}{n}\approx 1k$ times overhead just to avoid asynchronous training. Section~\ref{sec:Analyses} shows that asynchronous learning is effective enough and it is unnecessary to refresh the entire corpus's representation after each training batch.




\subsection{Analyses on ANCE Asynchronous Learning}
\label{sec:Analyses}
\input{Figures/fluct}

In this experiment we first analyze the main advantage of ANCE: stronger and more realistic negatives during training. Then we study the influence of delayed updates in the Asynchronous learning.



Figure~\ref{fig.neg overlap} shows the overlap of negatives used in training versus the negatives seen in actual dense retrieval in the testing stage, measured through the learning process on the same set sampled queries. 
% For each of these approaches, in each of \cx{TODO: XXX} training step, we 
Similar to the illustration in Figure~\ref{fig.motivation}, which is from the actual learned representations in ANCE(FirstP) on query ``what is the most popular food in Switzerland'', there is very low overlap between the training negatives, sampled from BM25 or Randomly, and the negatives seen in testing by their corresponding trained models. Only 11\% testing negatives appears in the BM25 negative pool and there is no overlap with the randomly sampled ones in training. The mismatch between training distribution and testing distribution risks optimizing DR models to undesired direction and perhaps was the main roadblock preventing DR to outperform sparse retrieval.

ANCE fundamentally eliminates this discrepancy by using the exact same approach in retrieval training instances and in testing. In the beginning of its training, as it is warmed up by BM25 Neg, ANCE already constructs negative instances with 60\% overlap. As the model converging, the ANCE negatives become closer to the testing negatives and eventually the two become the same, by definition. This is the sole difference between ANCE trained DR models with those DR baselines and itself alone elevates DR models outperform sparse retrieval in document ranking.

Figure~\ref{fig:fluct} illustrates the behavior of ANCE Asynchronous learning with different ANN index refreshing frequencies. When the refreshing rate is too low, the representation space used to construct training negatives is delayed too much from the up-to-date one being optimized. This leads to very fluctuating training curves and may even cause the model to diverge, e.g., in Figure~\ref{fig:fluct}.a, as the training distribution is too far away from optimal (though still better than not using ANCE negatives). As expected, refreshing the ANN index more frequently leads to much more smooth training curve, as shown in Figure~\ref{fig:fluct}.c., with the price of slower training speed. 
However, as shown in Figure~\ref{fig:fluct}.d, which is our choice, a 1:1 allocation of inferencer GPU and trainer GPU amounts is adequate to train the DR models effectively. More ablation studies of those hyper-parameter choices are included in Appendix.

In Appendix, we also include results in other retrieval tasks and examples of winning/losing queries of DR versus BM25. The t-SNE plots of all TREC DL evaluation queries, the same with Figure~\ref{fig.motivation}, and our intuitions on them are also included in Appendix.


==> ANCE/Arxiv/evaluation.tex <==
\section{Evaluation Results}
\input{Tables/doc_pass_combined}

\begin{figure}\hspace*{-3cm}\CenterFloatBoxes
   \begin{floatrow}
       \ffigbox[\FBwidth]{\raisebox{-1\height}{\includegraphics[width=0.65\columnwidth]{Figures/overlap_line.pdf}}}{\caption{Training Neg Overlap vs Final KNN}\label{Dinah}}
        \ttabbox{\resizebox{0.45\textwidth}{!}{\input{Tables/efficiency_inference_tbl}}
         }{\caption{Efficiency of ANCE Inference and Training}\label{mytable}}
   \end{floatrow}
\end{figure}


\begin{figure}[htbp]
  \centering
  \hspace*{-1.5cm}\includesvg[width=1.2\columnwidth]{Figures/fluctuation.svg}
  \caption{ANCE learning fluctuation study}
\end{figure}



\subsection{Text Retrieval Effectiveness}

\cx{Results showing our performance gain over previous baselines in TREC Doc and passage ranking
\begin{enumerate}
    \item BM25
    \item Best BM25 + query expansion
    \item feature-based LeToR
    \item DeepCT
    \item BERT-Siamese (Zhuyun's paper)
    % \item reranking results of Roberta on ANCE and BM25 \lx{you mean retrieval? or reranking?}
\end{enumerate}
Also show inference time of these work.
}


\lx{checked with Chenyan, we will need that for document first} \cx{Yes and then paragraph.}




\cx{Results compare our training methods with other negative sampling. 
\begin{enumerate}
    \item Random negative
    \item in batch NCE
    \item BM25 negative
    \item BM25 warm up + in batch NCE
    \item BM25 + IB (FAIR paper)
    \item [TODO] BM25 warm up + Momentum NCE
\end{enumerate}
}
%  \ja{Should we show a comparison where we pick hard negatives just in one iteration Vs picking in multiple steps for convergence; most training exercises pick negatives once and here we say that picking it for every N step and then converging N steps is superior}
% }


\subsection{Dense Retrieval and ANCE learning Efficiency}
\cx{
o	A table measure the efficiency of the following on the document retrieval task, in our final setting:
	Time for sparse retrieval (BM25) per query (100 doc)
	Time of BERT Reranking (rerank top 100 of BM25)
	Time of dense retrieval (100 doc)
	The time cost in refreshing the ANN index in ANCE training, breaking down to:
•	ANN refreshing, including:
o	Time to infer the representation of the corpus
o	Time to build the ANN index
•	Batch training:
o	Time to fetch the top K (k=the number we used in the final model) negatives from ANN for each training batch
o	The time cost per training batch
}




\subsection{ANCE Learning Analyses}
\label{sec:ancenegatives}

% \begin{figure}
%     \centering
%     \input{Figures/fluctuation.svg}
% \end{figure}






% \input{Tables/efficiency_training_tbl}

\cx{Figures to show the negative overlaps of BM25 Neg, Rand Neg, ANCE neg, Versus ANN inference time negatives along the training curve of ANCE and BM25+Rand Neg}

\cx{Zoom in the ANCE learning process and demonstrate why ANCE is crucial and what is its effect in the learning process.
\begin{enumerate}
    \item Show the paired training loss curve and testing performance along the curve
    \item track and show the overlap of the ANCE negatives and BM25 negatives along the curve. Show the overlap and testing NDCG in these data points a) the overlap in the beginning of ANN refresh; b) in the middle between ANN refresh.
    \item also compare the negative overlap with in batch negatives (that there is very little overlap)
    \item compare the negative overlap at the end of each ANN refresh, show that the model learns stronger and stronger negatives. Also show the positive recall in top K of ANN at those data points \lx{I think end of each refresh basically means using query-inference from the beginning of next start checkpoint, but using doc inference from the previous checkpoint} \cx{query inference from the beginning of next start checkpoint is almost the same at the end of past checkpoint as they are only one backprop away?}
    \item \ao{is there any difference in learning speed, i.e. does ANCE help get the model to perform better faster or does it to allow training longer or both? \cx{Compared to which baseline? On doc, in batch negative or random all hurt, and just can't learn much, ANCE I think quickly passes them and far ahead. We can compare with BM25+IB (FAIR paper) on passage I think. TODO Lee: what is their learn curve look like? \ao{I was thinking to compare with BM25+IB}}}
\end{enumerate}}

\subsection{Case Studies}
\begin{figure}[tb]
  \centering
  \hspace*{-0.5cm}\includegraphics[width=1.2\columnwidth]{Figures/case_studies.pdf}
  \caption{Winning & Losing Case\lx{moving to native latex table below Table 4} }
\end{figure}

\input{Tables/case_study_tbl}

\cx{Show the wining cases and losing cases of ANN retrieval VS BM25. 
\begin{enumerate}
    \item  Plot the per query win/loss VS BM25 (the same style as in TREC DL Overview paper Figure 2 (this might leave in appendix)
    \item show winning case and losing examples of each
    \item \ao{what is our hole rate? are the holes good/bad, should we study this a bit? \cx{I think we can show it but as we are better than baseline I think we don't need to spend much time to study the hole rate, showing that we are better even with holes is good enough? \ao{sure, I'm just interested what the hole rate is and if it's large there might be something interesting}}}
\end{enumerate}
}






==> ANCE/Arxiv/intro_v1.tex <==
\section{Introduction}



Many language systems rely on text retrieval to find relevant information  for later stages. For example,
search ranking~\cite{nogueira2019passage}, open domain question answering~\cite{chen2017reading}, and fact verification~\cite{yang2018hotpotqa, thorne2018fact} all first use text retrieval to find relevant information as the input to their later stage ranking, QA, and reasoning models.
All these later stage models enjoy the effectiveness from deep learning techniques~\cite{rajpurkar2016squad, wang2018glue}, while, in contrast, the first stage retrieval is still largely exact matching discrete bag-of-words~\cite{chen2017reading, zhaotransxh2020, yang2018hotpotqa, nogueira2019passage}.
Such sparse retrieval, e.g., BM25~\cite{bm25}, has various intrinsic challenges, i.e., vocabulary mismatch~\cite{croft2010search}, and leads to noises or missed information challenging or even impossible to recover in later stages~\cite{craswell2020overview, luan2020sparsedense, yang2018hotpotqa}


% The noisy and incomplete information brought in by the sparse first retrieval, limits the full potential of modern language AI systems, as t
% which brings in and missed information
% BM25~\cite{bm25}, unsupervised sparse retrieval using hand-crafted rules, is still a strong baseline and sometimes even the state-of-the-art, 40 years after its invention~\cite{zamani2018neural, karpukhin2020dense, luan2020sparsedense, lee2019latent}.
% The limited capability of the sparse first retrieval enforces a potential upper bound of modern language AI systems.
% The intrinsic challenge of sparse retrieval, i.e. vocabulary mismatch and language varieties~\cite{croft2010search}, brings in noisy and missed information in the first stage, which is challenging, sometimes impossible 
% for the later deep neural models to recover~\cite{yang2018hotpotqa, craswell2020overview}. 




% \cx{The importance of dense retrieval:
% \begin{enumerate}
%     \item resolve the bottleneck in e2e information system
%     \item unleash the full potential of neural methods in many downstream applications
%     \item unified and easier to maintain infrastructure
%     \item Also Pretrained LM and ANN inference are getting ready
% \end{enumerate}
% }
% \cx{The observations and challenges in recent progress:
% \begin{enumerate}
%     \item good for short passage but not as good on longer passage
%     \item reranking is promising but not yet fully e2e retrieval, many times have to combine with sparse model
%     \item even some permissive analyses that the capacity of encoding has to be very high for documents
% \end{enumerate}
% }

Dense retrieval (DR), which retrieves texts using learned distributed representations, is a promising potential direction to overcome this sparse retrieval bottleneck~\cite{lee2019latent, chang2020pre, luan2020sparsedense, gao2020complementing, ma2020zero, dhingra2020differentiable, karpukhin2020dense}: The representation space is fully learnable and can leverage the strength of pretraining, while the retrieval operation is sufficiently efficient thanks to the recent progress in Approximate Nearest Neighbor (ANN) search~\cite{johnson2019billion}.
One would expect dense retrieval to revolutionize the first stage retrieval, as deep learning has done in almost all language tasks, which, However, is not yet the case: Recent studies often found that dense retrieval with even pretrained language models under performs with BM25, especially on long texts~\cite{luan2020sparsedense, lee2019latent}, and DR is often used in combination and as an add-on to BM25~\cite{gao2020complementing, ma2020zero}.
The underwhelming performance even raises concerns whether it is reasonable to encoding the entire document into one dense vector~\cite{luan2020sparsedense}.
% , and the effectiveness of dense retrieval is mainly when combined with spare retrieval~\cite{gao2020complementing, ma2020zero}---as an add-on to BM25, but not yet a next-gen retrieval.

\input{Figures/motivation}



% \cx{Our solution:
% \begin{enumerate}
%     \item We identified the main bottleneck is actually in the training phrase, the mismatch between negatives seem in training and ANN inference
%     \item Developed a new training mechanism in the NCE framework, but instead of in-batch sampling, we directly do that in ANN, which is exact how the dense retrieval model is to be used
% \end{enumerate}
% }

In this paper we identify the main reason of such underwhelming performance of dense retrieval, especially on longer texts, is the learning part. Specifically, the mismatches of negatives sampled for training and the actually negatives in retrieval. 
% \ja{Previous sentence and next sentence are both technically strong and convey vital aspect of understanding; consider : Too many commas, suggest breaking down the long sentence for better readability}
In training, the negatives is either randomly sampled, selected in nearby batches, or from the sparse retrieval, following standard learning to rank settings~\cite{liu2009learning}. However, when testing, the trained model needs to retrieve the relevant documents in the entire corpus, e.g., via ANN, which is drastically different  from the negatives in sparse retrieval nor the random sampled negatives can provide the minutiae required for ranking among the top retrievals ($\mathsection$~\ref{sec:Analyses}). 


% \cx{More details of ANCE:
% \begin{enumerate}
%     \item We build ANN index with the doc representations
%     \item directly pick negatives from the ANN for each q and d+ label
%     \item refresh ANN after certain steps, as asynchronous updates
%     \item until converges in validation
% \end{enumerate}
% }

We eliminate this mismatch with Approximate nearest neighbor Noise Contrastive Estimation (ANCE), which follows the principle of NCE~\cite{gutmann2010noise, mnih2013learning, oord2018representation}, and selects stronger, \textit{more realistic}, negatives from an ANN index in learning. The ANN index includes the encodings of the documents/passages, from the same representation model being learned for the dense retrieval, and is parallelly updated and asynchronously refreshed as the optimization goes on. The negatives are sampled from this ANN index using the same retrieval function (dot product, e.g.), the same representation model (though delayed due to the asynchronous index update). 
This provides much stronger and more realistic negative instances---exactly the same as the retrieval model will face in inference time---and eliminate the discrepancy in the representation learning and testing.





% \cx{Our contribution as shown in experiments:
% \begin{enumerate}
%     \item The first to outperform all sparse retrieval, BM25 and beyond, as well as feature-based LeToR on TREC DL Doc task, a realistic, large scale, document retrieval task from Bing queries and documents.  
%     \item stronger than other training mechanisms: NCE, in batch, BM25+NCE, etc. (hopefully also momentum).
%     \item All with vanilla BERT-Siamese,  works for both doc ranking and passage ranking, with simple max-pooling or longformer on doc side.
% \end{enumerate}
% }

In TREC Deep Learning Track's large scale document and passage ranking benchmarks~\cite{craswell2020overview}, ANCE significantly boost the retrieval accuracy of dense retrieval. With ANCE training, the vanilla BERT-Siamese dual encoder, the same architecture used in several parallel research~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}, significantly outperforms all dense retrieval baselines, many with same architecture but different training scheme, sparse retrieval methods, including BM25 and many upgraded variations, and even the two-stage retrieval and reranking state-of-the-art IR pipeline which uses BERT as the neural ranker.  
We found the later very impressive: the dot-product retrieval in the ANCE learned representation space provides more effective, more efficiency, and simpler solution than the existing state-of-the-art two-stage IR pipeline.
% the ANCE-learned model is a simple dot-product operation in the learned representation space, 
% it not only improves the effectiveness, but also simplifies and speeds up the system's pipeline.

This overwhelming performance is the first we have observed in dense retrieval.
In our studies we show how the negatives from sparse retrieval or other sampling method differ from the negatives dense retrieval models face in testing, and how ANCE fundamentally resolves this difference.
% the actual dense retrieval 
% and our analyses provide further insights and illustrate how ANCE effectively optimizes the representation for simpler and more accurate dense retrieval.
We also show how the ANN index refreshing influences the ANCE training and the necessity of fast asynchronous refreshing to keep the representations in the index on-pace with the representation being optimized. We plan to make our implementation of ANCE training and the asynchronous refreshing of ANN index publicly available to facilitate future research in representation learning. 




% \cx{Our insights:
% \begin{enumerate}
%     \item the main gain is from our ANCE training, without it, there is a clear gap in reranking and retrieval, and our analyses show how the gap of different negatives are resolved during the ANCE training.
%     \item More details in how/when to refresh index, the LR scheduling, warm up, and negative sampling, to shine lights of representation learning in other related tasks
%     \item case studies to show the different behavior of dense retrieval and sparse retrieval 
% \end{enumerate}
% }

==> ANCE/Arxiv/openqair.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cccc|cccc} \hline \hline
         &   \multicolumn{4}{c|}{\textbf{Single Task Training}} 
         & \multicolumn{4}{c}{\textbf{Multi Task Training}}  \\ \hline
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c|}{\textbf{TriviaQA}} 
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c}{\textbf{TriviaQA}}  \\ \hline
         \textbf{Retriever} 
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100} \\ \hline
        BM25 & 59.1 & 73.7 & 66.9 & 76.7 & -- & -- & -- & -- 
        \\ 
        DPR & 78.4 & 85.4 & 79.4& 85.0 & 79.4 & 86.0 & 78.8 & 84.7 
        \\
        BM25 + DPR & 76.6 & 83.8 & 79.8 & 84.5 &  78.0 & 83.9 & 79.9 & 84.4
        \\ \hline
        ANCE & \textbf{81.9} & \textbf{87.5} & \textbf{80.3} & \textbf{85.3} & \textbf{82.1} & \textbf{87.9} & \textbf{80.3} & \textbf{85.2} \\
        \hline 
    \end{tabular}
% \end{table}

==> ANCE/Arxiv/p_res.tex <==
\lx{this is placeholder template until numbers are fully replaced}
\begin{table*}[ht]
    \centering
    \small

        \begin{tabular}{l|cc|cc|cc} \hline \hline
    & \multicolumn{2}{c|}{\textbf{MARCO Dev}} 
    & \multicolumn{2}{c|}{\textbf{TREC Rerank}} 
    & \multicolumn{2}{c}{\textbf{TREC Retrieval}}
    \\ \hline  
           \textbf{Method}     
    &  \textbf{MRR@10} &  \textbf{Recall@1k}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
    \\ \hline
    
{BM25}
& 0.20 &  ~ & ~ & ~ & ~ 
\\\hline
DeepCT~\cite{dai2019context} & Copy marco number and leave passage ones as n.a.\\ 
{TREC Best Retrieval}  & \\
{TREC Best Trad} &  \\
{Bert Ranker}  
& -- & -- & ~ & -- & -- & -- 
\\ \hline
{\textbf{Sentence-Bert}} & ~ & ~ & ~ & ~ & ~ & ~  \\
{w/ BM25 negative} 
& 0.299 & 0.928 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ NCE} 
& 0.256 & 0.943 & ~ & ~ & ~ & ~
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ IB} 
& 0.261 & 0.949 & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ BM25 + IB} 
& 0.311 & 0.952 & ~ & ~ & ~ & ~  \\ % mnt/semi/kwtang/msmarco/20200506_1937_nll_first_ln_9579aec6-2b94-400a-99d9-70b287a8e86c/checkpoint-90000/
\hline
{\textbf{Warmup from BM25}} & ~ & ~ & ~ & ~ & ~ & ~  \\

{w/ NCE} 
& 0.279 & 0.942 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ IB} 
& 0.280 & 0.948 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

%{w/ IB + BM25} 
%& ~ & ~ & ~ & ~ & ~ & ~ 
%\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ ANCE} & \textbf{0.330} & \textbf{0.959} & ~ & ~ & ~ & ~  \\ %../../../../glue_data/MSMarcoANN/rdot_clf_nll_4gpu_768d_t200_highlr_continue_with_2x_refresh/checkpoint-65000

\hline \hline
    \end{tabular}
     \caption{TREC DL Track 2019 Passage 
    \label{tab:passage_overal}}
\end{table*}



==> ANCE/Arxiv/related.tex <==
\section{Related Work}

% \cx{NeurIR starts with representation based model: CDSSM~\cite{huang2013learning}, but later interaction-based are strong with cross attention~\cite{guo2016deep}, especially with relevance specific representations~\cite{xiong2017knrm}. BERT performs well in interaction model~\cite{nogueira2019passage} but the study how dense retrieval with BERT is just started.
% }

% \cx{Related work in dense retrieval: 
% Dense retrieval in OpenQA~\cite{lee2019latent}.
% Mix-batch NCE and BM25~\cite{karpukhin2020dense}.
% ReQA~\cite{ahmad2019reqa} and pretraining study of dense retrieval~\cite{chang2020pre}.
% The use of ANN dense retrieval in QA and pretraining: REALM~\cite{guu2020realm} and Reasoning~\cite{dhingra2020differentiable}.
% Recent parallel work that have to combine dense and sparse: empirical study~\cite{ma2020zero}, learn with sparse~\cite{gao2020complementing}, theory analyses and combination~\cite{luan2020sparsedense}.
% }

In neural information retrieval (Neu-IR), neural ranking models are categorized into representation-based and interaction-based, depending on whether they represent query and document separately, or model the detailed interactions between term pairs~\cite{guo2016deep}.
For example, BERT ranker~\cite{nogueira2019passage} takes the concatenated query-document sequence and models the term interactions with self-attention, thus is interaction-based, while BERT-Siamese is representation-based. 
Previous research found interaction-based models more effective then representation-based, that modeling the interaction between discrete query-document term pairs seemed a necessity~\cite{xiong2017knrm, dai2019deeper, qiao2019understanding}. \ao{sentence}


However, the advantage of interaction-based Neu-IR is only directly applicable in the reranking stage, as for each query, the model needs to know the to-be-scored candidate documents, which require a first-stage sparse retrieval to provide. To break this sparse retrieval bottleneck, researchers revisited the representation-based model with BERT for dense retrieval, leading to a series of progresses including the BERT dual-encoder latent retrieval in OpenQA~\cite{lee2019latent}, the ReQA OpenQA dense retrieval benchmark~\cite{ahmad2019reqa}, and customized pretraining for it~\cite{chang2020pre}, etc.
Nevertheless, especially in long document retrieval, the effectiveness of dense retrieval alone was underwhelming, that it has to be combined with, and serves as an ``add-on'' to, sparse retrieval~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}; \ao{sentence} it was unclear whether it is possible to encode the entire document into one dense vector without losing too much information~\cite{luan2020sparsedense}.


Using Noise Constructive Estimation~\cite{gutmann2010noise, mnih2013learning} to construct stronger negative training instances are mostly recently by the contrastive representation learning framework in computer vision, for example, InfoNCE~\cite{oord2018representation}, SimCLR~\cite{chen2020simple}, and MoCo~\cite{he2019momentum, chen2020improved}. \ao{sentence} 
% More recently, in visual representation learning, MoCo improves InfoNCE and  constructs the negatives from a maintained queue of previous batches, using momentum updates to keep the representations in the queue up-to-date~\cite{he2019momentum, chen2020improved}. 
The technical choices in visual representation learning is different with in language, as language contains a natural ``dictionary''~\cite{he2019momentum}: NCE upon sampled random negatives is not as effective in learning language representations~\cite{karpukhin2020dense}. \ao{sentence}
Technical-wise, refreshing the ANN index in parallel has been recently utilized in REALM, where it is used to fetch contexts as input to the grounded language model, instead of as contrastive learning instances~\cite{guu2020realm}.
% ANCE can be viewed as natural next step of InfoNCE and MoCo with more global negatives from the ANN index of the entire corpus. This is supported by the asynchronous ANN refreshing with the representation learning, which has been recently utilized by REALM,
% though they use ANN to fetch contexts as input to the grounded language model, instead of as contrastive learning instances~\cite{guu2020realm}.




% With ANCE we demonstrate that 1) BERT-Siamese, the representation-based Neu-IR model, matches the effectiveness in the reranking setting with the BERT ranker, the interaction-based model, without requiring any term level interaction in the sparse representations; 2) dense retrieval, in the ANCE learned representation space, outperform the state-of-the-art sparse retrieval by itself, and nearly matches the accuracy of the cascade pipeline, while being much simpler and efficient.  



% Recently, similar ideas have been visited extensively in representation learning, for example, InfoNCE uses NCE to pick images that to contrast the representation of the image~\cite{oord2018representation}, and is a core component in the SimCLR framework for contrastive visual representation learning~\cite{chen2020simple}. MoCo improves InfoNCE and constructs the negatives by maintaining a queue of previous batches and their representations, which use momentum updates to keep a smooth encoding~\cite{he2019momentum, chen2020improved}. 








==> ANCE/Conclusion.tex <==
\section{Conclusion}


% ANCE fundamentally eliminates the discrepancy between the representation learning of texts and their usages in dense retrieval.
% Our ANCE trained dense retrieval model, the vanilla BERT-Siamese, convincingly outperforms all dense retrieval and sparse retrieval baselines in our large scale document retrieval and passage retrieval experiments.
% It nearly matches the ranking accuracy of the state-of-the-art cascade sparse retrieval and BERT reranking pipeline.
% More importantly, all these advantages are achieved with a standard transformer encoder at a 1\% online inference latency, using a simple dot-product in the ANCE-learned representation space.

In this paper, we first provide theoretical analyses on the convergence of representation learning in dense retrieval. 
We show that under common conditions in text retrieval, the local negatives used in DR training are uninformative, yield low gradient norms, and contribute little to the learning convergence.
We then propose ANCE to eliminate this bottleneck by constructing training negatives globally from the entire corpus.
Our experiments demonstrate the advantage of ANCE in web search, OpenQA, and the production system of a commercial search engine.
Our studies empirically validate our theory that ANCE negatives have much bigger gradient norms, reduce the stochastic gradient variance, and improve training convergence.




==> ANCE/Convergence.tex <==
\section{Analyses on The Convergence of Dense Retrieval Training}
\label{sec:theory}


In this section, we provide theoretical analyses on the convergence of representation training in dense retrieval.
% Using the variance reduction framework~\citep{alain2015variance, katharopoulos2018not}, 
We first show the connections between learning convergence and gradient norms, then the bounded gradient norms by uninformative negatives, and finally, how in-batch local negatives are ineffective under common conditions in dense retrieval.

\textbf{Convergence Rate and Gradient Norms:} Let $l(d^+, d^-)=l(f(q, d^+), f(q, d^-)$ be the loss function on the training triple $(q, d^+, d^-)$, $P_{D^-}$ the  negative sampling distribution for the given $(q, d^+)$, and $p_{d^-}$ the sampling probability of negative instance $d^-$, a stochastic gradient decent (SGD) step with importance sampling~\citep{alain2015variance} is:
\begin{align}
    \theta_{t+1} &= \theta_t - \eta \frac{1}{Np_{d^-}} \nabla_{\theta_t} l(d^+, d^-), \label{eq:wsgd}
\end{align}
with $\theta_t$ the parameter at $t$-th step, $\theta_{t+1}$ the one after, and $N$ the total number of negatives. The scaling factor $\frac{1}{Np_{d^-}}$ is to make sure Eqn.~\ref{eq:wsgd} is an unbiased estimator of the full gradient.

Then we can characterize the converge rate of this SGD step as the movement to optimal $\theta^*$. Following derivations in variance reduction~\citep{katharopoulos2018not, johnson2018training}, let $g_{d^-}= \frac{1}{Np_{d^-}} \nabla_{\theta_t} l(d^+, d^-)$ the weighted gradient, the convergence rate is:
\begin{align}
    \E\Delta^t &= ||\theta_t - \theta^*||^2 - \E_{P_{D^-}}(||\theta_{t+1} - \theta^* ||^2) \\
    % &= ||\theta_t||^2 - 2\theta_t^T\theta^* + ||\theta^*||^2 - E_{P_{D-}}(||\theta_{t+1}||^2) + 2 \theta^{*T}E_{P_{D-}}(\theta_{t+1}) - ||\theta^*||^2 \\
    &= ||\theta_t||^2 - 2\theta_t^T\theta^*  - \E_{P_{D^-}}(||\theta_{t}-\eta g_{d^-}||^2) + 2 \theta^{*T}\E_{P_{D^-}}(\theta_{t}-\eta g_{d^-}) \\
    &= -\eta^2\E_{P_{D^-}}(||g_{d^-}||^2) + 2 \eta \theta_t^T \E_{P_{D^-}}(g_{d^-}) - 2\eta \theta^{*T}\E_{P_{D^-}}(g_{d^-}) \\
    &= 2\eta \E_{P_{D^-}}(g_{d^-})^T (\theta_t - \theta^*) -\eta^2\E_{P_{D^-}}(||g_{d^-}||^2) \\
    &= 2\eta \E_{P_{D^-}}(g_{d^-})^T (\theta_t - \theta^*) -\eta^2\E_{P_{D^-}}(g_{d^-})^T \E_{P_{D^-}}(g_{d^-}) - \eta^2 \text{Tr}(\mathcal{V}_{P_{D^-}}(g_{d^-})). \label{eqn:variance}
\end{align}
This shows we can obtain better convergence rate by sampling from a distribution $P_{D^-}$ that minimizes the variance of the gradient estimator, $\E_{P_{D^-}}(||g_{d^-}||^2)$, or $\text{Tr}(\mathcal{V}_{P_{D^-}}(g_{d^-}))$ as the estimator is unbiased. There exists an optimal distribution that: 
\begin{align}
    p^*_{d^-} = \text{argmin}_{p_{d^-}} \text{Tr}(\mathcal{V}_{P_{D^-}}(g_{d^-})) \propto ||\nabla_{\theta_t} l(d^+, d^-)||_2, \label{eqn.oracle}
\end{align}
which is to sample proportionally to per instance gradient norm.
This is a well known result in importance sampling~\citep{alain2015variance, johnson2018training}. It can be proved by applying Jensen's inequality on the gradient variance and then verifying that Eqn.~\ref{eqn.oracle} achieves the minimum. We do not repeat this proof and refer to~\citet{johnson2018training} for exact derivations. 

Intuitively, an negative instance with larger gradient norm is more likely to reduce the training loss more, while those with diminishing gradients are not informative. Empirically, the correlation of gradient norm and training convergence is also observed in BERT fine-tuning~\citep{mosbach2020stability}.

\textbf{Diminishing Gradients of Uninformative Negatives:}
The oracle distribution in Eqn.~\ref{eqn.oracle} is too expensive to compute and the closed form of gradient norms can be complicated in  deep neural networks.
Nevertheless, for MLP networks, \citet{katharopoulos2018not} derives an upper bound of the per sample gradient norm:
\begin{align}
     ||\nabla_{\theta_t} l(d^+, d^-)||_2  \leq L \rho || \nabla_{\phi_L} l(d^+, d^-) ||_2,
\end{align}
where L is the number of layers, $\rho$ is composed by pre-activation weights and gradients in intermediate layers, and  $|| \nabla_{\phi_L} l(d^+, d^-) ||_2$ is the gradient w.r.t. the last layer.
Intuitively, the intermediate layers are more regulated by various normalization techniques; the main moving piece is $|| \nabla_{\phi_L} l(d^+, d^-) ||_2$~\citep{katharopoulos2018not}. 

For common learning to rank loss functions, for example, BCE loss and pairwise hinge loss, we can verified that~\citep{katharopoulos2018not}:
\begin{align}
    l(d^+, d^-) \rightarrow 0 \Rightarrow  || \nabla_{\phi_L} l(d^+, d^-) ||_2 \rightarrow 0 \Rightarrow ||\nabla_{\theta_t} l(d^+, d^-)||_2  \rightarrow 0. \label{eqn.lossbound}
\end{align}
Intuitively, negative samples with near zero loss have near zero gradients and contribute little to model convergence.
The convergence of dense retrieval model training relies on the informativeness of constructed negatives.

\textbf{Inefficacy of Local In-Batch Negatives:} We argue that the in-batch local negatives are unlikely to provide informative samples due to two common properties of text retrieval.

Let $D^{-*}$ be the set of informative negatives that are hard to distinguish from $D^{+}$, and $b$ be the batch size, we have (1) $b \ll |C|$, the batch size is far smaller than the corpus size; (2) $|D^{-*}| \ll |C|$, that only a few negatives are informative and the majority of corpus is trivially unrelated. 

Both conditions are easy to verify empirically in dense retrieval benchmarks.
The two together make the probability that a random mini-batch includes meaningful negatives $p=\frac{b |D^{-*}|}{|C|^2}$ close to zero. Selecting negatives from local training batches is unlikely to provide optimal training signals for dense retrieval. 















==> ANCE/Evaluation.tex <==
\input{Tables/doc_pass_combined}
\input{Tables/joint}
% \input{Tables/openqa_retrieval_full}
% \input{Tables/floatprod} 

\section{Evaluation Results}


In this section, we first evaluate the effectiveness and efficiency of ANCE. Then we empirically study the convergence of ANCE training following our theoretical analyses.
% When its convergence.

\subsection{Effectiveness and Efficiency}
\label{sec:efficiency}



The results on TREC 2019 DL benchmark are in Table~\ref{tab:overall}. ANCE significantly outperforms all sparse retrieval, including DeepCT, which uses BERT to learn term weights~\citep{dai2019transformer}. 
Among all different negative construction mechanisms, ANCE is the only one that elevates BERT-Siamese to robustly exceed the sparse methods in document retrieval.
It also outperforms DPR in passage retrieval in OpenQA (Table~\ref{tab:openqa}).
ANCE's effectiveness is even more observed in real production (Table~\ref{tab.prod}) with about 15\% relative gains all around.
Its better retrieval does indeed lead to better answer accuracy with the same readers used in RAG~\citep{lewis2020retrieval} and DPR (Table~\ref{tab.qae2e}). 
% , where switching to ANCE training improves a production model stably by around 15\%.
% much bigger corpora and more efficiency constraints.



\input{Tables/efficiency_qa}
\input{Figures/dotprod}
\input{Figures/lossnorm}

Among all DR models, ANCE has the smallest gap between its retrieval and reranking accuracy, showing the importance of global negatives in training retrieval models. 
ANCE retrieval nearly matches the accuracy of the cascade IR with interaction-based BERT Reranker.
This overthrows a previously-held belief that modeling term-level interactions is necessary in search~\citep{xiong2017knrm, qiao2019understanding}. 
\textit{With ANCE, we can learn a representation space that effectively captures the finesse of search relevance.} 








Table~\ref{tab.efficiency} measures the efficiency ANCE (FirstP) in TREC DL document retrieval. The online latency is on one query and 100 retrieved documents.
% Note the exact numbers depends on the computing environment.
DR with standard batching provides a \textit{100x speed up compared to BERT Rerank}, a natural benefit from the Siamese network and pre-computable document encoding. 
In ANCE training, the bulk of computing is to update the encodings of the training corpus using new checkpoints.
Assuming the model used to sample negatives and to be learned is the same, this is inevitable but can be mitigated by asynchronous index refresh.




\subsection{Empirical Analyses on Training Convergence}
\label{sec:Analyses}



% This experiment empirically verifies our theories on the learning convergence of dense retrieval.



We first show the long tail distribution of search relevance in dense retrieval. As plotted in Fig.~\ref{fig:dotprod}, there are a few instances per query with significant higher retrieval scores, while the majority form a long tail. 
In retrieval/ranking, the key challenge is to distinguish the relevant ones among those highest scored ones; the rest is trivially irrelevant. We also empirically measure the probability of local in-batch negatives including informative negatives ($D^{-*}$), by their overlap with top 100 highest scored negatives. 
This probability, either using NCE Neg or Rand Neg, is \textit{zero}, the same as our theory assumes. 
In comparison, the overlap between BM25 Neg with top DR retrieved negatives is 15\%, while  that of ANCE negatives starts at 63\% and converges to 100\% by design.

Then we empirically validate our theory that local negatives lead to lower loss, bounded gradient norm, and thus slow convergence.
The training loss and pre-clip gradient norms during DR training are plotted in Fig.~\ref{fig:gradnorm}. As expected, the uninformative local negatives are trivial to separate, yielding near-zero training loss, while ANCE global negatives are much harder and maintain a high training loss. 
The same with our theoretical assumption, the gradient norms of local negatives are indeed restricted closely to zero. In comparison, the gradient norms on ANCE global negatives are bigger by orders of magnitude. This confirms ANCE better approximates the oracle importance sampling distribution $ p^*_{d^-} \propto ||\nabla_{\theta_t} l(d^+, d^-)||_2$ and improves learning convergence.


\subsection{Discussions}

We use BERT-Siamese and NLL loss to be consistent with recent research. We have experimented with cosine similarity and BCE/hinge loss, where we observe even smaller gradient norms on local negatives. But the retrieval accuracy is not much better.
We include additional experiments in Appendix. \ref{app:hole} discusses the surprisingly small overlap (<25\%) between dense retrieval results and sparse retrieval results. DR is a fundamentally different approach and more studies are required to understand its behavior. 
\ref{app:lap} and~\ref{app:ablation} study the asynchronous gaps and hyperparameters. 
% In general ANCE is quit robust and we stick to standard hyperparameter settings.
\ref{app:case} includes case studies that the irrelevant documents from ANCE are often still ``semantically related'' and very different from those made by sparse retrieval.
% where errors are more because of matched query terms in unrelated documents.


==> ANCE/Experiment.tex <==
\section{Experimental Methodologies}
\label{sec:exp}
This section describes our experimental setups. More details can be found in Appendix~\ref{app:exp} and~\ref{app:hole}.



\textbf{Benchmarks:} 
The web search experiments use the TREC 2019 Deep Learning (DL) Track benchmark~\citep{craswell2020overview}, a large scale ad hoc retrieval dataset. 
We follow the official guideline and evaluate mainly in the retrieval setting, but also results when reranking top 100 BM25 candidates.
% are reranked.
% reranking accuracy using top 100 candidates from BM25.


% (more in Appendix~\ref{app:exp} and~\ref{app:hole}). 

The OpenQA experiments use the Natural Questions (NQ)~\citep{kwiatkowski2019natural} and TriviaQA (TQA)~\citep{joshi2017triviaqa}, following the exact settings from \citet{karpukhin2020dense}.
% \footnote{https://github.com/facebookresearch/DPR.}. 
The metrics are Coverage@20/100, which evaluate whether the Top-20/100 retrieved passages include the answer. We also evaluate whether ANCE's better retrieval can propagate to better answer accuracy, by running the state-of-the-art systems' readers on top of ANCE instead of DPR retrieval. The readers are RAG-Token~\citep{lewis2020retrieval} on NQ and DPR Reader on TQA, in their suggested settings.

We also study the effectiveness of ANCE in the first stage retrieval of a commercial search engine's production system. We change the training of a production-quality DR model to ANCE, and evaluate the offline gains in various corpus sizes, encoding dimensions, and exact/approximate search.

\textbf{Baselines:} In TREC DL, we include best runs in relevant categories and refer to \citet{craswell2020overview} for more baseline scores. We implement recent DR baselines that use the same BERT-Siamese, but vary in negative construction: random sampling in batch (Rand Neg), random sampling from BM25 top 100 (BM25 Neg)~\citep{lee2019latent, gao2020complementing} and the 1:1 combination of BM25 and Random negatives (BM25 + Rand Neg)~\citep{karpukhin2020dense, luan2020sparsedense}. We also compare with contrastive learning/Noise Contrastive Estimation, which uses hardest negatives in batch (NCE Neg)~\citep{gutmann2010noise, oord2018representation, chen2020simple}.
In OpenQA, we compare with DPR, BM25, and their combinations~\citep{karpukhin2020dense}.





\textbf{Implementation Details:} 
In TREC DL, recent research found MARCO passage training labels cleaner~\citep{yanidst} and BM25 negatives can help train dense retrieval~\citep{karpukhin2020dense, luan2020sparsedense}. 
Thus, we include a ``BM25 Warm Up'' setting (BM25 $\rightarrow *$), where the DR models are first trained using MARCO official BM25 Negatives. ANCE is also warmed up by BM25 negatives. All DR models in TREC DL are fine-tuned from RoBERTa base~\citep{liu2019roberta}.
In OpenQA, we warm up ANCE using the released DPR checkpoints~\citep{karpukhin2020dense}.

 To fit long documents in BERT-Siamese, ANCE uses the two settings from \citet{dai2019deeper}, FirstP which uses the first 512 tokens of the document, and MaxP, where the document is split to 512-token passages (maximum 4) and the passage level scores are max-pooled. The max-pooling operation is natively supported in ANN.
The ANN search uses the Faiss IndexFlatIP Index~\citep{johnson2019billion}.
We use 1:1 Trainer:Inference GPU allocation,  index refreshing per 10k training batches, batch size 8, and gradient accumulation step 2 on 4 GPUs. For each positive, we uniformly sample one negative from ANN top 200.
We measured ANCE efficiency using a single 32GB V100 GPU, on a cloud VM with Intel(R) Xeon(R) Platinum 8168 CPU and 650GB of RAM memory.

% More experimental details can be found in Appendix~\ref{app:exp} and our upcoming code release.


==> ANCE/Figures/dotprod.tex <==
\begin{figure}[t]
    \centering
        \subfigure[ANCE FirstP (100\%) \label{fig:a1}]{\includegraphics[scale=0.27]{Figures/ANCE.pdf}} \hspace{1mm}
        \subfigure[NCE Neg (0\%)\label{fig:b1}
        ]{\includegraphics[scale=0.27]{Figures/BM25_NCE.pdf}} \hspace{1mm}
        \subfigure[Rand Neg (0\%) \label{fig:c1}
        ]{\includegraphics[scale=0.27]{Figures/BM25_Rand.pdf}} \hspace{1mm}
        \subfigure[BM25+Rand (7\%)\label{fig:d1}      ]{\includegraphics[scale=0.27]{Figures/BM25_BM25_Rand.pdf}} \vspace{-0.6cm}
        \caption{ 
        The top DR scores for 10 random TREC DL testing queries. The x-axes are their ranking order. The y-axes are their retrieval scores minus corpus average.
        All models are warmed up by BM25 Neg. 
        The percentages are the overlaps between the testing and training negatives near convergence.
        \label{fig:dotprod}
        }
\end{figure} 

==> ANCE/Figures/fluct.tex <==

\begin{figure}[t]
    \centering
        \subfigure[10k Batch; 4:4; 1e-5\label{fig:a}]{\includegraphics[scale=0.27]{Figures/lrplot_0.pdf}}
        \subfigure[20k Batch; 8:4; 1e-6\label{fig:b}
        ]{\includegraphics[scale=0.27]{Figures/lrplot_1.pdf}}
        \subfigure[5k Batch; 4:8; 1e-6\label{fig:c}
        ]{\includegraphics[scale=0.27]{Figures/lrplot_2.pdf}}
        \subfigure[10k Batch; 4:4; 5e-6\label{fig:d}      ]{\includegraphics[scale=0.27]{Figures/lrplot_3.pdf}}
        \caption{
        Training loss and testing NDCG of ANCE (FirstP) on documents, with different ANN index refreshing (e.g., per 10k Batch), Trainer:Inferencer GPU allocation, and learning rate (e.g., 1e-5). X-axes is the training steps in thousands.
        \label{fig:fluct}
        }
\end{figure} 




==> ANCE/Figures/lossnorm.tex <==

\begin{figure}[t]
    \centering
        \subfigure[Training Loss\label{fig:a2}      ]{\includegraphics[scale=0.27]{Figures/Loss.pdf}} \hspace{1mm}
        \subfigure[Grad Norm (Bottom) \label{fig:b2}]{\includegraphics[scale=0.27]{Figures/First.pdf}} 
        \hspace{1mm}
        \subfigure[Grad Norm (Middle)\label{fig:c2}
        ]{\includegraphics[scale=0.27]{Figures/Middle.pdf}} \hspace{1mm}
        \subfigure[Grad Norm (Top)\label{fig:d2}
        ]{\includegraphics[scale=0.27]{Figures/Last.pdf}} 
        \vspace{-0.6cm}
        \caption{The loss and gradient norms during DR training (after BM25 warm up). The gradient norms are on the bottom (1-4), middle (5-8), and top (9-12) BERT layers. 
        The x-axes are training steps. 
        \label{fig:gradnorm}
        }
\end{figure} 

==> ANCE/Figures/motivation.tex <==

% \cx{Outlines. Each bracket is }
\begin{wrapfigure}{tr}{0.4\linewidth}
% \vspace{-0.5cm}
  \centering
  \includegraphics[width=\columnwidth]{Figures/tsne_case.pdf}
  \caption{T-SNE~\citep{maaten2008visualizing} representations of query, relevant documents, negative training instances from BM25 (BM25 Neg) or randomly sampled (Rand Neg), and testing negatives (DR Neg) in dense retrieval.\vspace{-0.5cm}
~\label{fig.motivation} 
}

\end{wrapfigure}

==> ANCE/Impact.tex <==
\section*{Broader Impact}
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}


 For the past decades, in academic community we have been joking that every year we made 10\% progress upon BM25, but it had always been 10\% upon the same BM25; the techniques developed require more and more IR domain knowledge that might be unfamiliar to researchers in other related fields. For example, in OpenQA, document retrieval was often done with vanilla BM25 instead of the well-tuned BM25F, query expansion, or SDM.
In industry, many places build their search solutions upon open source solutions, such as Lucene and ElasticSearch, where BM25, a technique invented in the 1970s and 1980s, was incorporated as late as 2015~\cite{elasticbm25}; the required expertise, complex infrastructure, and computing resource make many missing out the benefits of Neu-IR.


With their effectiveness, efficiency, and simplicity, ANCE and dense retrieval have the potential to redefine the next stage of information systems and provide broader impacts in many fronts.
% the following fronts.

\textbf{Empower User with Better Information Access:} The effectiveness of DR is particularly prominent for exploratory or knowledge acquisition information needs. 
Formulating good queries that have term overlap with the target documents often requires certain domain knowledge, which is a barrier for users trying to learn new information.
A medical expert trying to learn how to build a small search functionality on her patient's medical records may not be aware of the terminology ``BM25'' and ``Dense Retrieval''.
By matching user's information need and the target information in a learned representation space, ANCE has the potential to overcome this language barrier and empower users to achieve more in their daily interactions with search engines.


\textbf{Reduce Computing Cost and Energy Consumption in Neural Search Stack:}
The nature of dense retrieval makes it straightforward to conduct most of the costly operations offline and reuse the pre-computed document vectors.
This leads to 100x better efficiency and will significantly reduce the hardware cost and energy consumption needed when serving deep pretrained models online. We consider this a solid step towards carbon neutrality in the search stack.


\textbf{Democratize the Benefit of Neural Techniques:} Building, maintaining, and serving a cascade IR pipeline with the advanced pretrained models is daunting and may not lead to good ROI for many companies not in the web search business. In comparison, the simple dot product operation in a mostly pre-computed representation space is much more accessible. Faiss and many other libraries provide easy-to-access solution of efficient ANN retrieval; our (to be) released pretrained encoders and ANCE open-source solution will fill in the effectiveness part. Together we will democratize the recent revolutions in neural information retrieval to a much broader audience and end-users.

 



==> ANCE/Introduction.tex <==
\section{Introduction}


% \cx{Reduce this paragraph to half, and merge the 2nd para in to one paragraph that overviews the progress of Dense Retrieval.}
Many language systems rely on text retrieval as their first step to find relevant information.
For example, search ranking~\citep{nogueira2019passage}, open domain question answering (OpenQA)~\citep{chen2017reading}, and fact verification~\citep{thorne2018fact} all first retrieve relevant documents for their later stage reranking, machine reading, and reasoning models.
All these later-stage models enjoy the advancements of deep learning techniques~\citep{rajpurkar2016squad, wang2018glue}, while, the first stage retrieval still mainly relies on matching discrete bag-of-words, e.g., BM25, which has become the bottleneck of many systems~\citep{nogueira2019passage, luan2020sparsedense, zhaotransxh2020}.
%Due to intrinsic challenges such as vocabulary mismatch~\citep{croft2010search}, sparse retrieval inevitably introduces noisy information and often becomes the bottleneck of many systems~\citep{yang2018hotpotqa, luan2020sparsedense}. 


Dense Retrieval (DR) aims to overcome the sparse retrieval bottleneck by matching texts in a continuous representation space learned via deep neural networks~\citep{lee2019latent, karpukhin2020dense, luan2020sparsedense}.
It has many desired properties: fully learnable representation, easy integration with pretraining, and efficiency support from approximate nearest neighbor (ANN) search~\citep{johnson2019billion}. These make dense retrieval an intriguing potential choice to fundamentally overcome some intrinsic limitations of sparse retrieval, for example, vocabulary mismatch~\citep{croft2010search}.

A key challenge in DR is to construct proper negative instances during its representation learning~\citep{karpukhin2020dense}.
Unlike in reranking where negatives are naturally the irrelevant documents from previous retrieval stages, in first stage retrieval, DR models have to distinguish relevant documents from \textit{all irrelevant ones} in the entire corpus. As illustrated in Fig.~\ref{fig.motivation}, these \textit{global negatives} are quite different from negatives retrieved by sparse models. 
% \cx{discuss the NCE method in representation learning, how recent DR methods try them, and the still under performing situation.}

Recent research explored various ways to construct negative training instances for dense retrieval~\citep{huang2020embedding, karpukhin2020dense}., e.g., using contrastive learning~\citep{faghri2017vse++, oord2018representation, he2019momentum,  chen2020simple} to select hard negatives in current or recent mini-batches. 
However, as observed in recent research~\citep{karpukhin2020dense},
the in-batch local negatives, though effective in learning word or visual representations, are not significantly better than spare-retrieved negatives in representation learning for dense retrieval. In addition, the accuracy of dense retrieval models often underperform BM25, especially on documents~\citep{lee2019latent, gao2020complementing,luan2020sparsedense}.





\input{Figures/motivation}

In this paper, we first theoretically analyze the convergence of dense retrieval training with negative sampling.
% present the theoretical analysis  negative instance construction in dense retrieval.
Using the variance reduction framework~\citep{alain2015variance, katharopoulos2018not},
we show that, under conditions commonly met in dense retrieval, local in-batch negatives lead to diminishing gradient norms, resulted in high stochastic gradient variances and slow training convergence --- the local negative sampling is the bottleneck of dense retrieval's effectiveness.




Based on our analysis, we propose Approximate nearest neighbor Negative Contrastive Estimation (ANCE), a new contrastive representation learning mechanism for dense retrieval.
Instead of random or in-batch local negatives, ANCE constructs global negatives using the being-optimized DR model to retrieve from the entire corpus.
This fundamentally aligns the distribution of negative samples in training and of irrelevant documents to separate in testing.
From the variance reduction point of view, these ANCE negatives lift the upper bound of per instance gradient norm, reduce the variance of the stochastic gradient estimation, and lead to faster learning convergence.

% This fundamentally eliminates the discrepancy between the negative instances used to train DR models and the irrelevant documents those models face when deployed. Our theoretical analysis also suggests 
% that the ANCE negatives have bigger gradient norms and lead to faster convergence.



We implement ANCE using an asynchronously updated ANN index of the corpus representation. Similar to \citet{guu2020realm}, we maintain an Inferencer that parallelly computes the document encodings with a recent checkpoint from the being optimized DR model, and refresh the ANN index used for negative sampling once it finishes, to keep up with the model training.
% to keep up with the model training.
% Once the entire corpus is encoded, the inferencer refresh the ANN index to construct more up-to-date ANCE negatives that asynchronously keep up with the model training process.
% This implementation only requires trainer-inference communication through shared file system and can be employed in any contrastive learning scenarios.
Our experiments demonstrate the advantage of ANCE in three text retrieval scenarios: standard web search~\citep{craswell2020overview}, OpenQA~\citep{rajpurkar2016squad, kwiatkowski2019natural}, and in a commercial search engine's retrieval system. 
% In all scenarios, the vanilla BERT-Siamese DR model, trained by ANCE, outperforms not only all previous dense retrieval models but also state-of-the-art pretraining based sparse retrieval models. 
We also empirically validate our theory that the gradient norms on ANCE sampled negatives are much bigger than local negatives and thus improve the convergence of dense retrieval models. Our code and trained models are available at \url{https://aka.ms/ance}.
% \footnote{Code and trained models are in the supplementary material and will be open-sourced.}



==> ANCE/Method.tex <==

\begin{figure}[tb]
  \centering
  \hspace*{-0cm}\includegraphics[width=0.8\columnwidth]{Figures/ance_training_diagramV1.pdf}
  \caption{ANCE Asynchronous Training. The Trainer learns the representation using negatives from the ANN index. The Inferencer uses a recent checkpoint to update the representation of documents in the corpus and once finished, refreshes the ANN index with most up-to-date encodings.
  }
  \label{fig.ANCE} 
\end{figure}

\section{Approximate Nearest Neighbor Noise Contrastive Estimation}





Our analyses show the importance, if not necessity, to construct negatives \textit{globally} from the corpus. In this section, we propose \textit{A}pproximate nearest neighbor \textit{N}egative \textit{C}ontrastive \textit{E}stimation, (ANCE), which selects negatives from the entire corpus using an asynchronously updated ANN index.

\textbf{ANCE} samples negatives from the top retrieved documents via the DR model from the ANN index:
\begin{align}
  & \theta^* = \text{argmin}_{\theta} \sum_q \sum_{d^+\in D^+} \sum_{d^- \in D^-_\text{ANCE}} l(f(q, d^+), f(q, d^-)), \label{eq.fullloss}
\end{align}
with $D^-_\text{ANCE} = \text{ANN}_{f(q, d)} \setminus D^+$ and $\text{ANN}_{f(q, d)}$ the top retrieved documents by $f()$ from the ANN index.
By definition, $D^-_\text{ANCE}$ are the hardest negatives for the current DR model: $D^-_\text{ANCE} \approx D^{-*}$. In theory, these more informative negatives have higher training loss, higher upper bound on the gradient norms, and will improve training convergence.

ANCE can be used to train any dense retrieval model. For simplicity, we use a simple set up in recent research~\citep{luan2020sparsedense} with BERT Siamese/Dual Encoder (shared between $q$ and $d$), dot product similarity, and negative log likelihood (NLL) loss.
% \begin{align}
% &f(q,d) = \text{BERT-Siamese}(q, d) = \text{BERT}(q)^T \text{BERT}(d), \\
% &l(f(q, d^+), f(q, d^-)) = \text{NLL}(f(q, d^+), f(q, d^-)),
% \end{align}
% which uses the standard BERT Siamese architecture, dot product similarity, and NLL loss.


\textbf{Asynchronous Index Refresh:} 
During stochastic training, the DR model $f()$ is updated each mini-batch. Maintaining an update-to-date ANN index to select fresh ANCE negatives is challenging, as the index update requires two operations: 1) \textit{Inference}: refresh the representations of all documents in the corpus with an updated DR model;  2) \textit{Index}: rebuild the ANN index using updated representations. Although \textit{Index} is efficient~\citep{johnson2019billion}, \textit{Inference} is too expensive to compute per batch as it requires a forward pass on the entire corpus which is much bigger than the training batch. 

Thus we implement an asynchronous index refresh similar to \citet{guu2020realm}, and update the ANN index once every  $m$ batches, i.e., with checkpoint $f_k$. As illustrated in Fig.~\ref{fig.ANCE}, besides the Trainer, we run an Inferencer that takes the latest checkpoint (e.g., $f_{k}$) and recomputes the encodings of the entire corpus. In parallel, the Trainer continues its stochastic learning using $D^-_{f_{k-1}}$ from $\text{ANN}_{f_{{k-1}}}$.  Once the corpus is re-encoded, Inferencer updates the ANN index ($\text{ANN}_{f_{k}}$) and feed it to the Trainer.

In this process, the ANCE negatives ($D^-_\text{ANCE}$) are asynchronously updated to ``catch up'' with the stochastic training. 
The gap between the ANN index and the DR model optimization depends on the allocation of computing resources between Trainer and Inferencer. 
Appendix~\ref{app:lap} shows an 1:1 GPU split is sufficient to minimize the influence of this gap.





==> ANCE/Preliminary.tex <==
\section{Preliminaries}
In this section, we discuss the preliminaries of dense retrieval and its representation learning.

\textbf{Task Definition:} Given a query $q$ and a corpus $C$, the first stage retrieval is to find a set of documents relevant to the query $D^+=\{d_1,...,d_i,...,d_n\}$ from $C$ ($|D^+| \ll |C|$), which then serve as input to later more complex models~\citep{croft2010search}.
Instead of using sparse term matches and inverted index, \textit{Dense Retrieval}  calculates the retrieval score $f()$ using similarities in a learned embedding space~\citep{lee2019latent, luan2020sparsedense, karpukhin2020dense}:
\begin{align}
    f(q, d) &= \text{sim}(g(q; \theta), g(d; \theta)),  \label{eq.f}
\end{align}
where $g()$ is the representation model that encodes the query or document to dense embeddings. The encoder parameter $\theta$ provides the main capacity, often fine-tuned from pretrained transformers, e.g., BERT~\citep{lee2019latent}. The similarity function (sim()) is often simply cosine or dot product, to leverage efficient ANN retrieval~\citep{johnson2019billion, guoaccelerating}. 



\textbf{Learning with Negative Sampling:} The effectiveness of DR resides in learning a good representation space that maps query and relevant documents together, while separating irrelevant ones. The learning of this representation often follows standard learning to rank~\citep{liu2009learning}: Given a query $q$, a set of relevant document $D^+$ and irrelevant ones $D^-$, find the best $\theta^*$ that:
\begin{align}
    \theta^* &= \text{argmin}_{\theta} \sum_{q} \sum_{d^+\in D^+} \sum_{d^- \in D^-} l(f(q, d^+), f(q, d^-)). \label{eq.baseloss}
\end{align}
The loss $l()$ can be binary cross entropy (BCE), hinge loss, or negative log likelihood (NLL). 

A unique challenge in dense retrieval, targeting first stage retrieval, is that the irrelevant documents to separate are from the entire corpus $(D^- = C \setminus D^+)$. 
This often leads to millions of negative instances, which have to be sampled in training: 
\begin{align}
    \theta^* &= \text{argmin}_{\theta} \sum_q \sum_{d^+\in D^+} \sum_{d^- \in \hat{D}^-} l(f(q, d^+), f(q, d^-)). \label{eq.basefullloss}
\end{align}

A natural choice is to sample negatives $\hat{D}^-$ from top documents retrieved by BM25. However, they may bias the DR model to merely learn sparse retrieval and do not elevate DR models much beyond BM25~\citep{luan2020sparsedense}.
Another way is to sample negatives in local mini-batches, e.g., as in contrastive learning~\citep{oord2018representation, chen2020simple}, however, these local negatives do not significantly outperform BM25 negatives~\citep{karpukhin2020dense, luan2020sparsedense}.










==> ANCE/RelatedWork.tex <==
\section{Related Work}


% more on how ANCE challenged the assumption in Neu-IR and opened new research space
In early research on neural information retrieval (Neu-IR)~\citep{mitra2018introduction}, a common belief was that the interaction models, those that specifically handle term level matches, are more effective though more expensive~\citep{guo2016deep, xiong2017knrm, nogueira2019passage}. 
Many techniques are developed to reduce their cost, for example, distillation~\citep{gao2020understanding} and caching~\citep{humeau2020poly, khattab2020colbert, macavaney2020efficient}. 
ANCE shows that a properly trained representation-based BERT-Siamese is in fact as effective as the interaction-based BERT ranker. This finding will motivate many new research explorations in Neu-IR.

Deep learning has been used to improve various components of sparse retrieval, for example,  term weighting~\citep{dai2019deeper}, query expansion~\citep{zheng2020bert}, and document expansion~\citep{nogueira2019document}. 
Dense Retrieval chooses a different path and conducts retrieval purely in the embedding space via ANN search~\citep{ lee2019latent,  chang2020pre, karpukhin2020dense, luan2020sparsedense}. This work demonstrates that a simple dense retrieval system can achieve SOTA accuracy, while also behaves dramatically different from classic retrieval. The recent advancement in dense retrieval may raise a new generation of search systems.


Recent research in contrastive representation learning also shows the benefits of sampling negatives from a larger candidate pool.
In computer vision, \citet{he2019momentum} decouple the negative sampling pool size with training batch size, by maintaining a negative candidate pool of recent batches and updating their representation with momentum. This enlarged negative pool significantly improves unsupervised visual representation learning~\citep{chen2020improved}.
A parallel work~\citep{xiong2020answering} improves DPR by sampling negatives from a memory bank~\citep{wu2018unsupervised} --- in which the representations of negative candidates are frozen so more candidates can be stored.
Instead of a bigger local pool, ANCE goes all the way along this trajectory and constructs negatives globally from the entire corpus, using an asynchronously updated ANN index.

Besides being a real world application itself, dense retrieval is also a core component in many other language systems, for example, to retrieval relevant information for grounded language models~\citep{khandelwal2019generalization, guu2020realm},  extractive/generative QA~\citep{karpukhin2020dense, lewis2020retrieval}, and fact verification~\citep{xiong2020answering}, or to find paraphrase pairs for pretraining~\citep{lewis2020pre}. There dense retrieval models are either frozen or optimized indirectly by signals from their end tasks.
ANCE is orthogonal with those lines of research and focuses on the representation learning for dense retrieval. Its better retrieval accuracy can benefit many language systems. 






==> ANCE/Tables/ablation_overall.tex <==
\begin{table*}[t]
    \centering
    \small
     \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|c|c} \hline \hline
    & \multicolumn{3}{c|}{\textbf{Hyperparameter}} 
    & \multicolumn{1}{c|}{\textbf{MARCO Dev Passage}} 
    & \multicolumn{1}{c}{\textbf{TREC DL Document}}
    \\ 
      & {\textbf{Learning rate}}
      & {\textbf{Top K Neg}}
      & {\textbf{Refresh (step)}}
      
      & {\textbf{Retrieval MRR@10}} 
      & {\textbf{Retrieval NDCG@10}} 
    \\ \hline
    
\textbf{Passage ANCE} 
& 1e-6 & 200 & 10k & \textbf{0.33} & -- \\
& 1e-6 & 500 & 10k & 0.31 & -- \\
& 2e-6 & 200 & 10k & 0.29 & -- \\
& 2e-7 & 500 & 20k & 0.303 & -- \\
& 2e-7 & 1000 & 20k & 0.302 & -- \\

\hline 
\textbf{Document ANCE} 
& 1e-5 & 100 & 10k & -- & 0.58 \\
& 1e-6 & 100 & 20k & -- & 0.59 \\
& 1e-6 & 100 & 5k & -- & 0.60 \\
& 5e-6 & 200 & 10k & -- & \textbf{0.614} \\
& 1e-6 & 200 & 10k & -- & 0.61 \\
\hline
    \end{tabular}}
     \caption{Results of several different hyperparameter configurations. ``Top K Neg'' lists the top k ANN retrieved candidates from which we sampled the ANCE negatives from.
     ~\label{tab:ablation}}
\end{table*}

% \\\hline
% {2x learning rate } 
% & 0.29 \\ %nll_rdot_clf_ann_n20_t200_768_4gpu_even_higherlr Korean-DLTS
% {0.5x refresh rate} 
% & 0.307 \\
% % nll_rdot_clf_ann_n20_t200_768_4gpu_higherlr Korean_dlts
% {Negative sample from top 500} 
% & 0.310 \\ 
% % nll_rdot_clf_ann_n20_t500_768_4gpu_higherlr_2x_refresh Korean-DLTS
% {0.5x refresh rate + 0.2x learning rate + sample from top 500*} 
% % this model is more conservative, shooting for most smooth learning curve but also converges the slowest. We terminated the run after ~100k steps as it is just too slow to converge
% & 0.303 \\
% % nll_rdot_clf_ann_n20_t500_768_4gpu 
% % http://azure-eastus-v100-32gb-worker-loixjf.eastus.cloudapp.azure.com:31636/

% {0.5x refresh rate + 0.2x learning rate + sample from top 1000*} 
% % this model is MOST conservative, shooting for most smooth learning curve but also converges the slowest. We terminated the run after ~100k steps as it is just too slow to converge
% & 0.302 \\
% % nll_rdot_clf_ann_n20_t1000_768_4gpu
% %http://azure-eastus-v100-32gb-worker-mvlybt.eastus.cloudapp.azure.com:31055/


==> ANCE/Tables/case_study_tbl.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|p{5cm}|p{5cm}}

 \hline\hline
   & \textbf{ANCE} 
    & \textbf{BM25}
    \\
     \hline
     

\textbf{Query:} &\multicolumn{2}{l} {qid (104861): Cost of interior concrete flooring}
\\ \hline
{Title:} &  Concrete network: Concrete Floor Cost & Pinterest: Types of Flooring \\ \hline
{DocNo:} &D293855  &D2692315  \\ \hline
{Snippet:} & For a concrete floor with a basic finish, you can expect to pay \$2 to \$12 per square foot… 
& 
Know About Hardwood Flooring And Its Types White Oak Floors Oak Flooring Laminate Flooring In Bathroom …  \\  \hline

{Ranking Position:} & 1 & 1 \\ \hline
{TREC Label:} & 3 (Very Relevant) & 0 (Irrelevant) \\ \hline
{NDCG@10:} & 0.86 & 0.15\\ \hline\hline

\textbf{Query:} &\multicolumn{2}{l} {qid (833860): What is the most popular food in Switzerland}
\\ \hline
{Title:} &  Wikipedia: Swiss cuisine & Answers.com: Most popular traditional food dishes of Mexico \\ \hline
{DocNo:} &D1927155   &D3192888   \\ \hline
{Snippet:} & Swiss cuisine bears witness to many regional influences, … Switzerland was historically a country of farmers, so traditional Swiss dishes tend not to be… 
& 
One of the most popular traditional Mexican deserts is a spongy cake … (in the related questions section) What is the most popular food dish in Switzerland?…  \\  \hline

{Ranking Position:} & 1 & 1 \\ \hline
{TREC Label:} & 3 (Very Relevant) & 0 (Irrelevant) \\ \hline
{NDCG@10:} & 0.90 & 0.14\\ \hline\hline

\textbf{Query:} &\multicolumn{2}{l} {qid (1106007): Define visceral}
\\ \hline
{Title:} &  Vocabulary.com: Visceral & Quizlet.com: A\&P EX3 autonomic 9-10 \\ \hline
{DocNo:} &D542828    &D830758    \\ \hline
{Snippet:} & When something's visceral, you feel it in your guts. A visceral feeling is intuitive — there might not be a rational explanation, but you feel that you know what's best… 
& 
Acetylcholine A neurotransmitter liberated by many peripheral nervous system neurons and some central nervous system neurons…  \\  \hline

{Ranking Position:} & 1 & 1 \\ \hline
{TREC Label:} & 3 (Very Relevant) & 0 (Irrelevant) \\ \hline
{NDCG@10:} & 0.80 & 0.14\\ \hline

\end{tabular}
\caption{Queries in the TREC 2019 DL Track Document Ranking Tasks where ANCE performs better than BM25. Snippets are  manually extracted. The documents in the first disagreed ranking position are shown, where on all examples ANCE won.
The NDCG@10 of ANCE and BM25 in the corresponding query is listed.}
\label{tab:win_case_study}
\end{table}


\begin{figure}[t]
    \centering
        \subfigure[104861: interior flooring cost. ]{\label{case_ConcreteFloor}\includegraphics[scale=0.285]{Figures/tsne_case_101.pdf}}
        \subfigure[833860: popular Swiss food]
        {\label{case_SwitzerlandFood}\includegraphics[scale=0.285]{Figures/tsne_case_12.pdf}}
        \subfigure[1106007: define visceral ]{\label{case_Visceral}\includegraphics[scale=0.285]{Figures/tsne_case_381.pdf}}
        \caption{t-SNE Plots for Winning Cases in Table \ref{tab:win_case_study}.
        \label{fig:t-SNE_win_case}
        }
\end{figure} 


\begin{table}[t]
\centering
\small
\begin{tabular}{l|p{5cm}|p{5cm}}

 \hline\hline
   & \textbf{ANCE} 
    & \textbf{BM25}
    \\
     \hline
     
\textbf{Query:} &\multicolumn{2}{l} {qid (182539): Example of monotonic function}
\\ \hline
{Title:} &  Wikipedia: Monotonic function & Explain Extended: Things SQL needs: sargability of monotonic functions \\ \hline
{DocNo:} &D510209   &D175960   \\ \hline
{Snippet:} & In mathematics, a monotonic function (or monotone function) is a function between ordered sets that preserves or reverses the given order... For example, if y=g(x) is strictly monotonic on the range [a,b] … 
& 
I'm going to write a series of articles about the things SQL needs to work faster and more efficienly…  \\  \hline

{Ranking Position:} & 1 & 1 \\ \hline
{TREC Label:} & 0 (Irrelevant) & 2 (Relevant) \\ \hline
{NDCG@10:} & 0.25 & 0.61\\ \hline\hline

\textbf{Query:} &\multicolumn{2}{l} {qid (1117099): What is a active margin}
\\ \hline
{Title:} &  Wikipedia: Margin (finance) & Yahoo Answer: What is the difference between passive and active continental margins \\ \hline
{DocNo:} &D166625    &D2907204    \\ \hline
{Snippet:} & In finance, margin is collateral that the holder of a financial instrument … 
& 
An active continental margin is found on the leading edge of the continent where …  \\  \hline

{Ranking Position:} & 2 & 2 \\ \hline
{TREC Label:} & 0 (Irrelevant) & 3 (Very Relevant) \\ \hline
{NDCG@10:} & 0.44 & 0.74\\ \hline\hline

\textbf{Query:} &\multicolumn{2}{l} {qid (1132213): How long to hold bow in yoga}
\\ \hline
{Title:} &  Yahoo Answer: How long should you hold a yoga pose for & yogaoutlet.com: How to do bow pose in yoga \\ \hline
{DocNo:} &D3043610     &D3378723   \\ \hline
{Snippet:} & so i've been doing yoga for a few weeks now and already notice that my flexiablity has increased drastically. …That depends on the posture itself … 
& 
Bow Pose is an intermediate yoga backbend that deeply opens the chest and the front of the body…Hold for up to 30 seconds …  \\  \hline

{Ranking Position:} & 3 & 3 \\ \hline
{TREC Label:} & 0 (Irrelevant) & 3 (Very Relevant) \\ \hline
{NDCG@10:} & 0.66 & 0.74\\ \hline\hline

\end{tabular}
\caption{Queries in the TREC 2019 DL Track Document Ranking Tasks where ANCE performs worse than BM25. Snippets are manually extracted. The documents in the first position where BM25 wins are shown. The NDCG@10 of ANCE and BM25 in the corresponding query is listed. Typos in the query are from the real web search queries in TREC.}
\label{tab:loss_case_study}
\end{table}

\begin{figure}[t]
    \centering
        \subfigure[182539: monotonic function
        % Training batch 20k per refresh, train:inference GPU 8:4, learning rate 1e-6
        ]{\label{case_MonotonicFunc}\includegraphics[scale=0.285]{Figures/tsne_case_22.pdf}}
        \subfigure[1117099: active margin
        % Training batch 10k per refresh, train:inference GPU 4:4, learning rate 5e-6
        ]{\label{case_ActiveMargin}\includegraphics[scale=0.285]{Figures/tsne_case_20.pdf}}
        \subfigure[1132213: yoga bow ]{\label{case_yoga}\includegraphics[scale=0.285]{Figures/tsne_case_211.pdf}}
        \caption{t-SNE Plots for Losing Cases in Table \ref{tab:loss_case_study}.
        \label{fig:t-SNE_loss_case}
        }
\end{figure} 


==> ANCE/Tables/doc_pass_combined.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|cc|cc|cc} \hline \hline
    & \multicolumn{2}{c|}{\textbf{MARCO Dev}} 
    & \multicolumn{2}{c|}{\textbf{TREC DL Passage}} 
    & \multicolumn{2}{c}{\textbf{TREC DL Document}}
    \\ 
    
      & \multicolumn{2}{c|}{\textbf{Passage Retrieval}} 
      & \multicolumn{2}{c|}{\textbf{NDCG@10}} 
      & \multicolumn{2}{c}{\textbf{NDCG@10}} 
    \\  \hline
    &  \textbf{MRR@10} &  \textbf{Recall@1k}
      & \textbf{Rerank} & \textbf{Retrieval}
     & \textbf{Rerank} & \textbf{Retrieval}
    \\ \hline
    
\textbf{Sparse \& Cascade IR}  &  &  &  &  & &  \\
{BM25}
& 0.240 & 0.814 & -- & 0.506 & -- & 0.519 \\
{Best DeepCT} & 0.243 & n.a. & -- & n.a. & -- & 0.554
\\
{Best TREC Trad Retrieval}
& 0.240 & n.a. & -- & 0.554 & -- & 0.549\\
% {Best TREC Trad LeToR}
% & -- & -- & 0.556 & --   & 0.561 & -- 
% \\ 
{BERT Reranker}  % from literature 
& 
--  & -- & \textbf{0.742} & -- & 0.646 & -- 
\\\hline

{\textbf{Dense Retrieval}}  &  &  &  &  & & \\
Rand Neg & 0.261 & 0.949 & 0.605 & 0.552 & 0.615 & 0.543 \\
NCE Neg & 0.256 & 0.943 & 0.602 & 0.539 & 0.618 & 0.542 \\
BM25 Neg & 0.299 & 0.928 & 0.664 & 0.591 & 0.626 & 0.529 \\
DPR (BM25 + Rand Neg) & 0.311 & 0.952 & 0.653 & 0.600 & 0.629 & 0.557
  \\
BM25 $\rightarrow$ Rand & 0.280 & 0.948 & 0.609 & 0.576 & 0.637 & 0.566 \\
BM25 $\rightarrow$ NCE Neg & 0.279 & 0.942 & 0.608 & 0.571 & 0.638 & 0.564 \\
BM25 $\rightarrow$ BM25 + Rand & 0.306 & 0.939 & 0.648 & 0.591 & 0.626 & 0.540 \\
\hline
{ANCE (FirstP)} & \textbf{0.330} & \textbf{0.959} & 0.677 & \textbf{0.648} & 0.641 & 0.615 \\ 
{ANCE (MaxP)} & -- & -- & -- & -- & \textbf{0.671} & \textbf{0.628} \\
\hline 
    \end{tabular}
     \caption{Results in TREC 2019 Deep Learning Track.
     Results not available are marked as ``n.a.'', not applicable are marked as ``--''. Best results in each category are marked bold. \vspace{-0.3cm}
\smallskip~\label{tab:overall}}
\end{table*}



==> ANCE/Tables/efficiency.tex <==

\begin{figure}\TopFloatBoxes


   \begin{floatrow}
    \ttabbox{\resizebox{0.5\textwidth}{!}
         {\input{Tables/efficiency_inference_tbl}}}
         {\caption{Efficiency of Offline and Online (per query and 100 documents) operations. 
         }
         \label{tab.efficiency}}
    \hspace{0.2cm}   
    
    \ttabbox{\resizebox{0.4\textwidth}{!}
     {\input{Tables/prod}}}
      {\caption{Offline gains in the first stage retrieval of a commercial search engine at different Corpus size, encoding Dimension, and dense Retrieval setting. 
    %   The gains are measured by adding ANCE to the same DR model.
    %   using the same training labels.
    %   , same training data, same pretraining starting point, with ANCE versus without ANCE.
      }
      \label{tab.prod}
      }
   
   \end{floatrow}
\end{figure}



==> ANCE/Tables/efficiency_inference_tbl.tex <==
% \begin{sbsfigure*}
% \centering
% \small
 %\resizebox{\linewidth}{!}{
\begin{tabular}{l|r|r} \hline \hline
\textbf{Operation} & \textbf{Offline}  & \textbf{Online } \\ \hline
    % {\textbf{Sparse \& Cascade IR }} & \\
    {BM25 Index Build} & 3h & --  \\
    {BM25 Retrieval} & -- & 37ms  \\
    {BERT Rerank} &-- & 1.15s  \\
    Sparse IR Total (BM25 + BERT)  &-- & \textbf{1.42s} \\ 
    \hline
    
    {\textbf{ANCE Inference}} & \\
    {Encoding of Corpus/Per doc} & 10h/4.5ms & -- \\
    Query Encoding & --& 2.6ms \\
    ANN Retrieval (batched q) &-- & {9ms}  \\
    Dense Retrieval Total &-- & \textbf{11.6ms} 
    \\\hline
    {\textbf{ANCE Training}} &  \\
    {Encoding of Corpus/Per doc} & 10h/4.5ms & -- \\
    {ANN Index Build} & 10s & -- \\
    {Neg Construction Per Batch} & 72ms  & -- \\
    {Back Propagation Per Batch} & 19ms & -- \\
    \hline
    \end{tabular} \vspace{-1cm}
% \end{sbsfigure*}



==> ANCE/Tables/efficiency_qa.tex <==

\begin{figure}\BottomFloatBoxes
   \begin{floatrow}
   
       \ttabbox{\resizebox{0.45\textwidth}{!}
         {\input{Tables/openqa_e2e}}}
         {  
           \caption{OpenQA Test Scores in Single Task Setting. ANCE+Reader switches the retrieve of a system from DPR to ANCE and keeps the same reading model, which is RAG-Token on Natural Questions (NQ) and DPR Reader on Trivia QA (TQA).  
      \label{tab.qae2e}\vspace{-0.2cm}
      } 
      }
    
    \ttabbox{\resizebox{0.5\textwidth}{!}
         {\input{Tables/efficiency_inference_tbl}}
        \caption{Efficiency of ANCE Search and Training.\label{tab.efficiency}\vspace{-0.3cm}
        }
        }
  
   
   \end{floatrow}
\end{figure}

==> ANCE/Tables/floatefficiency.tex <==
% \vspace{-1cm}\newlength{\oldintextsep}
\setlength{\oldintextsep}{\intextsep}
\setlength\intextsep{-1pt}
\begin{wraptable}{tr}{0.48\textwidth}
\resizebox{\textwidth}{!}{\input{Tables/efficiency_inference_tbl}
\caption{Efficiency of Sparse and Dense IR.\label{tab.efficiency}\vspace{-0.2cm}}
}
\end{wraptable}         

==> ANCE/Tables/floatprod.tex <==

\begin{wraptable}{r}{0.4\textwidth}
\small
\resizebox{\textwidth}{!}{\caption{Offline gains in the first stage retrieval of a commercial search engine at different Corpus size, encoding Dimension, and dense Retrieval setting. 
      \label{tab:prod}
  } \input{Tables/prod}}
\end{wraptable}

==> ANCE/Tables/hole.tex <==
\begin{table*}[t]
    \centering
    \small
     \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc} \hline \hline
    & \multicolumn{3}{c|}{\textbf{TREC DL Passage}} 
    & \multicolumn{3}{c}{\textbf{TREC DL Document}}
    \\ 
    \hline
    
  \textbf{Method}
  & \textbf{Recall@1K} & \textbf{Hole@10} & \textbf{Overlap w. BM25}
       & \textbf{Recall@100} & \textbf{Hole@10} & \textbf{Overlap w. BM25}
  \\  \hline
    BM25 &0.685 & 5.9\% & 100\% &0.387 &0.2\% & 100\% \\ 
    \hline
    BM25 Neg &0.569 &25.8\% &11.9\%  &0.217 &28.1\% &17.9\%  \\
    BM25 + Rand Neg  &0.662 &20.2\% &16.4\%  &0.240 &21.4\% &21.0\%  \\ \hline
    ANCE (FirstP) &0.661 &14.8\% &17.4\%  &0.266 &13.3\% &24.4\%  \\
    ANCE (MaxP) &- &- &-  &0.286 &11.9\% &24.9\%  \\ \hline
  \end{tabular}}
  \caption{Coverage of TREC 2019 DL Track labels on Dense Retrieval methods. Overlap with BM25 is calculated on top 100 retrieved documents.
  \label{tab:hole}}
\end{table*}

==> ANCE/Tables/joint.tex <==

\begin{figure}\TopFloatBoxes
   \begin{floatrow}
    \ttabbox{\resizebox{0.6\textwidth}{!}
         {\input{Tables/openqa}}}
         {  
         \caption{Retrieval results (Answer Coverage at Top-20/100) on 
         Natural Questions (NQ) and Trivial QA (TQA) in the setting from ~\citet{karpukhin2020dense}. \vspace{-0.35cm}
        %   All Models are trained using the same data splits.   
          \label{tab:openqa}}}
    % \hspace{0.2cm}   
        \ttabbox{\resizebox{0.35\textwidth}{!}
     {\input{Tables/prod}}}
      {\caption{Relative gains in the first stage retrieval of a commercial search engine. The gains are from changing the training of a production DR model to ANCE. \vspace{-0.123cm}
    %   , with everything else unchanged.
    %   f ANCE retrieval model in a commercial search environment. 
      \label{tab.prod}
          }
      }
   
   \end{floatrow}
\end{figure}


==> ANCE/Tables/openqa.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cc|cc} \hline \hline
         &   \multicolumn{2}{c|}{\textbf{Single Task}} 
         & \multicolumn{2}{c}{\textbf{Multi Task}}  \\ \hline
         
         & \multicolumn{1}{c}{\textbf{NQ}} 
         & \multicolumn{1}{c|}{\textbf{TQA}} 
         & \multicolumn{1}{c}{\textbf{NQ}} 
         & \multicolumn{1}{c}{\textbf{TQA}}  \\ \hline
         \textbf{Retriever} 
        &  {Top-20/100} 
        &  {Top-20/100}
        &  {Top-20/100}
        &  {Top-20/100} \\ \hline
        BM25 & 59.1/73.7 & 66.9/76.7 & --/-- & --/-- 
        \\ 
        DPR & 78.4/85.4 & 79.4/85.0 & 79.4/86.0 & 78.8/84.7 
        \\
        BM25+DPR & 76.6/83.8 & 79.8/84.5 &  78.0/83.9 & 79.9/84.4
        \\ \hline
        ANCE & \textbf{81.9}/\textbf{87.5} & \textbf{80.3}/\textbf{85.3} & \textbf{82.1}/\textbf{87.9} & \textbf{80.3}/\textbf{85.2} \\
        \hline 
    \end{tabular}
% \end{table}

==> ANCE/Tables/openqa_e2e.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cc} \hline \hline
    \small
         \textbf{Model} 
         & \multicolumn{1}{c}{\textbf{NQ}} 
         & \multicolumn{1}{c}{\textbf{TQA}}  \\ \hline
        T5-11B~\citep{roberts2020much} & 34.5 & -
        \\ 
        T5-11B + SSM~\citep{roberts2020much} & 36.6 & -
        \\
        REALM~\citep{guu2020realm} & 40.4 & -
        \\ \hline
        % BM25 & 32.6 & 52.4
        % \\
        DPR~\citep{karpukhin2020dense} & 41.5 & 56.8
        \\
        DPR + BM25~\citep{karpukhin2020dense} & 39.0 & 57.0
        % ANCE DPR & - &
        \\ 
        RAG-Token~\citep{lewis2020retrieval} & 44.1 & 55.2
        \\
        RAG-Sequence~\citep{lewis2020retrieval} & 44.5 & 56.1
        \\ \hline
        ANCE + Reader  & \textbf{46.0} &  \textbf{57.5}
        \\
        \hline 
    \end{tabular}
% \end{table}

==> ANCE/Tables/openqa_retrieval_full.tex <==
\begin{table}[t]
    \centering
    % \small
     \caption{Answer Coverage at Top-K on 
         Natural Questions (NQ) and Trivial QA (TQA) in the setting from ~\citet{karpukhin2020dense}. Top-5/10 baseline results are produced using their open-source code.    \label{tab:openqa} \vspace{-0.5mm}  
     } 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cccc} \hline \hline
         &   \multicolumn{4}{c|}{\textbf{Single Task}} 
         & \multicolumn{4}{c}{\textbf{Multi Task}}  \\ \hline
         
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c|}{\textbf{Trivia QA}} 
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c}{\textbf{Trivia QA}}  \\ \hline
         \textbf{Retriever} 
            &  {Top-5/10} 
        &  {Top-20/100}
        &  {Top-5/10}
        &  {Top-20/100} 
        &  {Top-5/10} 
        &  {Top-20/100}
        &  {Top-5/10}
        &  {Top-20/100} \\ \hline
        BM25 & 
        & 59.1/73.7 
        &
        & 66.9/76.7 
        &
        & --/-- 
        &
        & --/-- 
        \\ 
        DPR &  68.3/74.9
        & 78.4/85.4 
        & 70.9/75.7
        & 79.4/85.0 
        &
        & 79.4/86.0 
        &
        & 78.8/84.7 
        \\
        BM25+DPR & 
        & 76.6/83.8 
        &
        & 79.8/84.5 
        &
        &  78.0/83.9 
        &
        & 79.9/84.4
        \\ \hline
        ANCE &  \textbf{71.8}/\textbf{77.8}
        & \textbf{81.9}/\textbf{87.5} 
        & \textbf{72.3}/\textbf{76.5}
        & \textbf{80.3}/\textbf{85.3} 
        &
        & \textbf{82.1}/\textbf{87.9} 
        &
        & \textbf{80.3}/\textbf{85.2} \\
        \hline 
    \end{tabular}
    }
\end{table}

==> ANCE/Tables/openqa_topvals.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cccc} \hline \hline
         \multicolumn{1}{c}{Retriever}
         & \multicolumn{1}{c}{Top-5}
         & \multicolumn{1}{c}{Top-10}
         & \multicolumn{1}{c}{Top-20}
         & \multicolumn{1}{c}{Top-100} \\ \hline
        
        \textbf{NQ} & & & &
        \\
        DPR & 68.3 & 74.9 & 80.0 & 86.0
        \\ 
        ANCE & 71.8 & 77.8 & 81.9 & 87.5 
        \\ \hline
        \textbf{TQA} & & & &
        \\
        DPR & 70.9 & 75.7 & 79.4 & 85.0
        \\
        ANCE & 72.3 & 76.5 & 80.3 & 85.3
        \\ \hline 
    \end{tabular}
% \end{table}

==> ANCE/Tables/prod.tex <==
\begin{tabular}{rrr|r} \hline \hline
\textbf{Corpus Size} & \textbf{Dim} & \textbf{Search} &
\textbf{Gain}  
\\ \hline	
250 Million & 768 & KNN & +18.4\% \\
8 Billion & 64 & KNN & +14.2\% \\
8 Billion & 64 & ANN & +15.5\% \\ \hline 
% $\approx$10B & 64 & ANN+Sparse & +2.6\% \\ \hline \hline
\end{tabular}

==> ANCE/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> DPR/figures/ir_training_examples.tex <==
\begin{figure}[!t]
    \center
    \includegraphics[scale=0.4,trim=0 0 0 40, clip]{figures/ir_training_examples_fig.pdf}
    \caption{Retriever top-$k$ accuracy with different numbers of training examples used in our dense passage retriever vs BM25. The results are measured on the development set of Natural Questions. Our DPR trained using 1,000 examples already outperforms BM25. }
    \label{fig:ir-training-examples}
\end{figure}


==> DPR/sections/acknowledgments.tex <==
\section*{Acknowledgments}
We thank the anonymous reviewers for their helpful comments and suggestions. 

==> DPR/sections/background.tex <==

\section{Background}
\label{sec:background}



The problem of open-domain QA studied in this paper can be described as follows.  Given a factoid question, such as
``\emph{Who first voiced Meg on Family Guy?}" or ``\emph{Where was the 8th Dalai Lama born?}", a system is required
to answer it using a large corpus of diversified topics.
More specifically, we assume the extractive QA setting, in which the answer is restricted to a span appearing in one or more passages in the corpus.
Assume that our collection contains $D$ documents, $d_1, d_2, \cdots, d_D$.
We first split each of the documents into text passages of equal lengths as the basic retrieval units\footnote{The ideal size and boundary of a text passage are functions of both the retriever and reader. We also experimented with natural paragraphs in our preliminary trials and found that using fixed-length passages performs better in both retrieval and final QA accuracy, as observed by~\citet{wang2019multi}.}
and get $M$ total passages in our corpus $\mathcal{C} = \{p_1, p_2, \ldots, p_{M}\}$, where
each passage $p_i$ can be viewed as a sequence of tokens $w^{(i)}_1, w^{(i)}_2, \cdots, w^{(i)}_{|p_i|}$.
Given a question $q$, the task is to find a span $w^{(i)}_s, w^{(i)}_{s+1}, \cdots, w^{(i)}_{e}$
from one of the passages $p_i$ that can answer the question.
Notice that %
to cover a wide variety of domains, the corpus size %
can easily range from millions of documents (e.g., Wikipedia) to billions (e.g., the Web).
As a result, any open-domain QA system needs to include an efficient \emph{retriever} component that
can select a small set of relevant texts, before applying the reader to extract the answer~\cite{chen2017reading}.\footnote{Exceptions include~\cite{seo2019real} and~\cite{roberts2020much}, which \emph{retrieves} and \emph{generates} the answers, respectively.}
Formally speaking, a retriever $R:(q,\mathcal{C}) \rightarrow \mathcal{C_F}$ is a function that takes as input a question $q$ and a corpus $\mathcal{C}$ and returns
a much smaller \emph{filter set} of texts $\mathcal{C_F} \subset \mathcal{C}$, where $|\mathcal{C_F}| = k \ll |\mathcal{C}|$.  For a fixed $k$, a \emph{retriever} can be evaluated in isolation on \emph{top-k retrieval accuracy}, which is the fraction of questions for which $\mathcal{C_F}$ contains a span that answers the question.





==> DPR/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we demonstrated that dense retrieval can outperform and potentially replace the traditional sparse retrieval component in open-domain question answering. While a simple dual-encoder approach can be made to work surprisingly well, we showed that there are some critical ingredients to training a dense retriever successfully. Moreover, our empirical analysis and ablation studies indicate that more complex model frameworks or similarity functions do not necessarily provide additional values. As a result of improved retrieval performance, we obtained new state-of-the-art results on multiple open-domain question answering benchmarks.




==> DPR/sections/exp-passage.tex <==
\input{tables/retrieval-accuracy.tex}

\section{Experiments: Passage Retrieval}
\label{sec:exp-psg}

In this section, we evaluate the retrieval performance of our Dense Passage Retriever (\model/), along with analysis on
how its output differs from traditional retrieval methods, the effects of different training schemes and the run-time efficiency.

The \model/ model used in our main experiments is trained using the in-batch negative setting (Section~\ref{sec:training}) with a batch size of $128$ and one additional BM25 negative passage per question.
We trained the question and passage encoders for up to $40$ epochs for large datasets (NQ, TriviaQA, SQuAD) and $100$ epochs for small datasets (TREC, WQ), with a learning rate of $10^{-5}$ using Adam, linear scheduling with warm-up and dropout rate~$0.1$.

While it is good to have the flexibility to adapt the retriever to each dataset, it would also be desirable to obtain a single retriever that works well across the board. To this end, we train a \emph{multi}-dataset encoder by combining training data from all datasets excluding SQuAD.\footnote{SQuAD is limited to a small set of Wikipedia documents and thus introduces unwanted bias. We will discuss this issue more in Section~\ref{sec:retrieval_main_results}.} %
In addition to \model/, we also present the results of BM25, the traditional retrieval method\footnote{\href{https://lucene.apache.org/}{Lucene} implementation. BM25 parameters $b=0.4$ (document length normalization) and $k_1=0.9$ (term frequency scaling) are tuned using development sets.} and BM25+\model/, using a linear combination of their scores as the new ranking function. 
Specifically, we obtain two initial sets of top-2000 passages based on BM25 and DPR, respectively, and rerank the union of them using BM25($q$,$p$) + $\lambda \cdot \mathrm{sim}(q,p)$ as the ranking function. We used $\lambda=1.1$ based on the retrieval accuracy in the development set.





\subsection{Main Results}
\label{sec:retrieval_main_results}

Table~\ref{tab:qa_ir} compares different passage retrieval systems on five QA datasets, using the top-$k$ accuracy ($k \in \{20,100\}$).
With the exception of SQuAD, \model/ performs consistently better than BM25 on all datasets.  The gap is especially large when $k$ is small (e.g., 78.4\% vs. 59.1\% for top-20 accuracy on Natural Questions).
When training with multiple datasets, TREC, the smallest dataset of the five, benefits greatly from more training examples.  In contrast, Natural Questions and WebQuestions improve modestly and TriviaQA degrades slightly.
Results can be improved further in some cases by combining \model/ with BM25 in both single- and multi-dataset settings.

We conjecture that the lower performance on SQuAD is due to two reasons. First, the annotators wrote questions after seeing the passage.  As a result, there is a high lexical overlap between passages and questions, which gives BM25 a clear advantage.  Second, the data was collected from only 500+ Wikipedia articles and thus
the distribution of training examples is extremely biased, as argued previously by~\newcite{lee2019latent}.

\input{figures/ir_training_examples.tex}

\subsection{Ablation Study on Model Training}
\label{subsec:ablation-retrieval}

To understand further how different model training options affect the results, we conduct several additional experiments and discuss our findings below.

\paragraph{Sample efficiency}

We explore how many training examples are needed to achieve good passage retrieval performance. %
Figure~\ref{fig:ir-training-examples} illustrates the top-$k$ retrieval accuracy with respect to different numbers of training examples,
measured on the development set of Natural Questions.
As is shown, a dense passage retriever trained using only 1,000 examples already outperforms BM25. 
This suggests that with a general pretrained language model, it is possible to train a high-quality dense retriever with a small number of question--passage pairs.
Adding more training examples (from 1k to 59k) further improves the retrieval accuracy consistently.

\paragraph{In-batch negative training}
\label{sec:ir_ablation}
We test different training schemes on the development set of Natural Questions and summarize the results in Table~\ref{tab:ir-ablation}. 
The top block is the standard 1-of-$N$ training setting, where each question in the batch is paired with a positive passage and its own set of $n$ negative passages~(Eq.~\eqref{eq:training}).
We find that the choice of negatives --- random, BM25 or gold passages (positive passages from other questions) --- does not impact the top-$k$ accuracy much in this setting when $k \ge 20$.%




The middle bock is the in-batch negative training (Section~\ref{sec:training}) setting.
We find that using a similar configuration (7 gold negative passages), in-batch negative training improves the results substantially.
The key difference between the two is whether the gold negative passages come from the same batch or from the whole training set.
Effectively, in-batch negative training is an easy and memory-efficient way to reuse the negative examples already in the batch rather than creating new ones.
It produces more pairs and thus increases the number of training examples, which might contribute to the good model performance. 
As a result, accuracy consistently improves as the batch size grows.

Finally, we explore in-batch negative training with additional ``hard" negative passages that have high BM25 scores given the question, but do not contain the answer string (the bottom block). These additional passages are used as negative passages for all questions in the same batch.
We find that adding a single BM25 negative passage improves the result substantially while adding two does not help further.

\input{tables/ir-ablation.tex}

\paragraph{Impact of gold passages} %
\label{sec:pos_pass}
We use passages that match the gold contexts in the original datasets (when available) as positive examples (Section~\ref{sec:qa-datasets}).
Our experiments on Natural Questions show that switching to distantly-supervised passages (using the highest-ranked BM25 passage that contains the answer), has only a small impact: 1 point lower top-$k$ accuracy for retrieval. %
Appendix~\ref{sec:distant} contains more details.



\paragraph{Similarity and loss}
\label{sec:sim_loss}
Besides dot product, cosine and Euclidean L2 distance are also commonly used as decomposable similarity functions.
We test these alternatives and find that L2 performs comparable to dot product, and both of them are superior to cosine.
Similarly, in addition to negative log-likelihood, a popular option for ranking is triplet loss, which compares a positive passage and a negative one directly with respect to a question~\cite{burges2005learning}.
Our experiments show that using triplet loss does not affect the results much.
More details can be found in Appendix~\ref{sec:alt-sim}. %


\paragraph{Cross-dataset generalization}
One interesting question regarding \model/'s discriminative training is how much performance degradation it may suffer from a non-iid setting. In other words, can it still generalize well when directly applied to a different dataset without additional fine-tuning? To test the cross-dataset generalization, we train \model/ on Natural Questions only and test it directly on the smaller WebQuestions and CuratedTREC datasets. We find that \model/ generalizes well, with 3-5 points loss from the best performing fine-tuned model in top-20 retrieval accuracy (69.9/86.3 vs. 75.0/89.1 for WebQuestions and TREC, respectively), while still greatly outperforming the BM25 baseline (55.0/70.9).









\subsection{Qualitative Analysis}

Although \model/ performs better than BM25 in general, passages retrieved by these two methods differ qualitatively. 
Term-matching methods like BM25 are sensitive to highly selective keywords and phrases, while \model/ captures lexical variations or semantic relationships better.
See Appendix~\ref{sec:qual_ana} for examples and more discussion.


\subsection{Run-time Efficiency}
\label{sec:efficiency}

The main reason that we require a retrieval component for open-domain QA is to reduce the number of candidate passages that the reader needs to consider, which is crucial for answering user's questions in real-time.
We profiled the passage retrieval speed on a server with Intel Xeon CPU E5-2698 v4 @ 2.20GHz and 512GB memory.
With the help of FAISS in-memory index for real-valued vectors\footnote{FAISS configuration: we used HNSW index type on CPU, neighbors to store per node = 512, construction time search depth = 200,  search depth = 128.}, \model/ can be made incredibly efficient, processing 995.0 questions per second, returning top 100 passages per question.
In contrast, BM25/Lucene (implemented in Java, using file index) processes 23.7 questions per second per CPU thread.

On the other hand, the time required for building an index for dense vectors is much longer.
Computing dense embeddings on 21-million passages is resource intensive, but can be easily parallelized, taking roughly 8.8 hours on 8 GPUs.
However, building the FAISS index on 21-million vectors on a single server takes 8.5 hours.
In comparison, building an inverted index using Lucene is much cheaper and takes only about 30 minutes in total.

==> DPR/sections/exp-setup.tex <==

\section{Experimental Setup}
\label{sec:exp-setup}

In this section, we describe the data we used for experiments and the basic setup.


\subsection{Wikipedia Data Pre-processing}
\label{sec:wiki-preprocessing}

Following~\cite{lee2019latent}, we use the English Wikipedia dump from Dec.~20, 2018 as the source documents for answering questions.
We first apply the pre-processing code released in DrQA~\cite{chen2017reading} to extract the clean, text-portion of articles from the Wikipedia dump.
This step removes semi-structured data, such as tables, info-boxes, lists, as well as the disambiguation pages.
We then split each article into multiple, disjoint text blocks of 100 words as \emph{passages}, serving as our basic retrieval units, following~\cite{wang2019multi}, which results in 21,015,324 passages in the end.\footnote{However, \citet{wang2019multi} also propose splitting documents into overlapping passages, which we do not find advantageous compared to the non-overlapping version.}
Each passage is also prepended with the title of the Wikipedia article where the passage is from, along with an \ttt{[SEP]} token.%


\subsection{Question Answering Datasets}
\label{sec:qa-datasets}

We use the same five QA datasets and training/dev/testing splitting method as in previous work~\cite{lee2019latent}.
Below we briefly describe each dataset and refer readers to their paper for the details of data preparation.

\noindent
\textbf{Natural Questions (NQ)}~\cite{kwiatkowski2019natural} was designed for end-to-end question answering.
The questions were mined from real Google search queries and the answers were spans in Wikipedia articles identified by annotators.

\noindent
\textbf{TriviaQA}~\cite{joshi-etal-2017-triviaqa} contains a set of trivia questions with answers that were originally scraped from the Web.

\noindent
\textbf{WebQuestions (WQ)}~\cite{berant2013semantic} consists of questions selected using Google Suggest API, where the answers are entities in Freebase.

\noindent
\textbf{CuratedTREC (TREC)}~\cite{baudivs2015modeling} sources questions from TREC QA tracks as well as various Web sources
and is intended for open-domain QA from unstructured corpora.

\noindent
\textbf{SQuAD v1.1}~\cite{rajpurkar2016squad} is a popular benchmark dataset for reading comprehension.
Annotators were presented with a Wikipedia paragraph, and asked to write questions that could be answered from the given text.
Although SQuAD has been used previously for open-domain QA research, it is not ideal because many questions lack context in absence of the provided paragraph.
We still include it in our experiments for providing a fair comparison to previous work and we will discuss more in Section~\ref{sec:retrieval_main_results}.


\paragraph{Selection of positive passages} %

Because only pairs of questions and answers are provided in TREC, WebQuestions and TriviaQA\footnote{We use the unfiltered TriviaQA version and discard the noisy evidence documents mined from Bing.}, we use the highest-ranked passage from BM25 that contains the answer as the positive passage.  If none of the top 100 retrieved passages has the answer, the question will be discarded.
For SQuAD and Natural Questions, since the original passages have been split and processed differently than our pool of candidate passages, we match and replace each gold passage with the corresponding passage in the candidate pool.\footnote{The improvement of using gold contexts over passages that contain answers is small. See Section~\ref{sec:pos_pass} and Appendix~\ref{sec:distant}.}
We discard the questions when the matching is failed due to different Wikipedia versions or pre-processing.
Table~\ref{tab:split-stats} shows the number of questions in training/dev/test sets for all the datasets and the actual questions used for training the retriever.


\input{tables/split-stats.tex}


==> DPR/sections/intro.tex <==

\section{Introduction}

\label{sec:intro}


Open-domain question answering (QA)~\cite{voorhees1999trec} is a task that answers factoid questions using a large collection of documents.
While early QA systems are often complicated and consist of multiple components~(\citet{ferrucci2012introduction,moldovan2003performance}, \textit{inter alia}),
the advances of reading comprehension models suggest a much simplified two-stage framework: (1) a context \emph{retriever} first selects a small subset of passages where some of them contain the answer to the question, and then (2) a machine \emph{reader} can thoroughly examine the retrieved contexts and identify the correct answer~\cite{chen2017reading}.
Although reducing open-domain QA to machine reading is a very reasonable strategy, a huge performance degradation is often observed in practice\footnote{For instance,
the exact match score on SQuAD v1.1 drops from above 80\% to less than 40\%~\cite{yang2019end}.}, indicating the needs of improving retrieval.


Retrieval in open-domain QA %
is usually implemented using TF-IDF or BM25~\cite{robertson2009probabilistic}, which matches keywords efficiently with an inverted index and can be seen
as representing the question and context in high-dimensional, sparse vectors (with weighting).
Conversely, the \emph{dense}, latent semantic encoding is \emph{complementary} to sparse representations by design.
For example, synonyms or paraphrases
that consist of completely different tokens may still be mapped to vectors close to each other.
Consider the question \ti{``Who is the bad guy in lord of the rings?''}, which can be answered from the context
\ti{``Sala Baker is best known for portraying the villain Sauron in the Lord of the Rings trilogy.''}
A term-based system would have difficulty retrieving such a context, while a dense retrieval system would be able to better match \ti{``bad guy''} with \ti{``villain''}
and fetch the correct context.
Dense encodings are also \emph{learnable} by adjusting the embedding functions, which provides additional flexibility to have a task-specific representation. With special in-memory data structures and indexing schemes, retrieval can be done efficiently using maximum inner product search (MIPS) algorithms~(e.g.,~\citet{NIPS2014_5329, guo2016quantization}).




However, it is generally believed that learning a good dense vector representation needs a large number of labeled pairs of question and contexts.
Dense retrieval methods have thus never be shown to outperform TF-IDF/BM25 for open-domain QA before ORQA~\cite{lee2019latent}, which proposes a sophisticated inverse cloze task (ICT) objective, predicting the blocks that contain the masked sentence, for additional pretraining.
The question encoder and the reader model are then fine-tuned using pairs of questions and answers jointly. %
Although ORQA successfully demonstrates that dense retrieval can outperform BM25, setting new state-of-the-art results on multiple open-domain QA datasets,
it also suffers from two weaknesses.
First, ICT pretraining is computationally intensive and it is not completely clear that regular sentences are good surrogates of questions in the objective function.
Second, because the context encoder is not fine-tuned using pairs of questions and answers, the corresponding representations could be suboptimal.


In this paper, we address the question: can we train a better dense embedding model using only pairs of questions and passages (or answers), \emph{without} additional pretraining?
By leveraging the now standard BERT pretrained model~\cite{devlin2018bert} and a dual-encoder architecture~\cite{bromley1994signature}, we focus on developing the right training scheme using a relatively small number of question and passage pairs. %
Through a series of careful ablation studies, our final solution is surprisingly simple: the embedding is optimized for maximizing inner products of the question and relevant passage vectors, with an objective comparing all pairs of questions and passages in a batch.
Our \emph{Dense Passage Retriever} (DPR) is exceptionally strong. It not only outperforms BM25 by a large margin (65.2\% vs. 42.9\% in Top-5 accuracy), but also results in a substantial improvement on the end-to-end QA accuracy compared to ORQA (41.5\% vs. 33.3\%) in the open Natural Questions setting~\cite{lee2019latent,kwiatkowski2019natural}.


Our contributions are twofold.
First, we demonstrate that with the proper training setup, simply fine-tuning the question and passage encoders on existing question-passage pairs
is sufficient to greatly outperform BM25.
Our empirical results also suggest that additional pretraining may not be needed.
Second, we verify that, in the context of open-domain question answering, a higher retrieval precision indeed translates to a higher end-to-end QA accuracy.
By applying a modern reader model to the top retrieved passages, we achieve comparable or better results on multiple QA datasets in the open-retrieval setting,
compared to several, much complicated systems.




==> DPR/sections/related.tex <==


\section{Related Work}
\label{sec:related}


Passage retrieval has been %
an important component for open-domain QA~\cite{voorhees1999trec}.
It not only effectively reduces the search space for answer extraction, but also identifies the support context for users to verify the answer.
Strong sparse vector space models like TF-IDF or BM25 have been used as the standard method applied broadly to various QA tasks~\citep[e.g.,][]{chen2017reading, yang2019end, Yang2019Data, nie2019revealing, min2019discrete, wolfson2020break}.
Augmenting text-based retrieval with external structured information, such as knowledge graph and Wikipedia hyperlinks, has also been explored recently~\cite{min2019knowledge,asai2020learning}.


The use of dense vector representations for retrieval has a long history since Latent Semantic Analysis~\cite{deerwester1990indexing}.
Using labeled pairs of queries and documents, discriminatively trained dense encoders have become popular recently~\cite{yih2011learning, huang2013learning, gillick-etal-2019-learning}, with applications to cross-lingual document retrieval, ad relevance prediction, Web search and entity retrieval. Such approaches complement the sparse vector methods as they can potentially give high similarity scores to semantically relevant text pairs, even without exact token matching. The dense representation alone, however, is typically inferior to the sparse one.
While not the focus of this work, dense representations from pretrained models, along with cross-attention mechanisms, have also been shown effective in passage or dialogue re-ranking tasks~\cite{nogueira2019passage,humeau2020poly}. 
Finally, a concurrent work~\cite{khattab2020colbert} demonstrates the feasibility of full dense retrieval in IR tasks. Instead of employing the dual-encoder framework, they introduced a late-interaction operator on top of the BERT encoders.






Dense retrieval for open-domain QA has been explored by~\citet{das2019multi}, who propose to retrieve relevant passages iteratively using reformulated question vectors.
As an alternative approach that skips passage retrieval, \citet{seo2019real} propose to encode candidate answer phrases as vectors and directly retrieve the answers to the input questions efficiently.
Using additional pretraining with the objective that matches surrogates of questions and relevant passages, \citet{lee2019latent} jointly train the question encoder and reader.
Their approach outperforms the BM25 plus reader paradigm on multiple open-domain QA datasets in QA accuracy, and is further extended by REALM~\cite{guu2020realm}, which includes tuning the passage encoder asynchronously by re-indexing the passages during training.
The pretraining objective has also recently been improved by \citet{Xiong2020ProgressivelyPD}.
In contrast, our model provides a simple and yet effective solution that shows stronger empirical performance, without relying on additional pretraining or complex joint training schemes.

\model/ has also been used as an important module in very recent work. For instance, extending the idea of leveraging hard negatives, \citet{Xiong2020ANCE} use the retrieval model trained in the previous iteration to discover new negatives and construct a different set of examples in each training iteration. Starting from our trained \model/ model, they show that the retrieval performance can be further improved. Recent work~\cite{Izacard2020fid, lewis2020rag} have also shown that DPR can be combined with generation models such as BART~\cite{lewis-etal-2020-bart} and T5~\cite{raffel2019T5}, achieving good performance on open-domain QA and other knowledge-intensive tasks.






==> DPR/sections/retriever.tex <==

\section{Dense Passage Retriever (\model/)}
\label{sec:retriever}


We focus our research in this work on improving the \emph{retrieval} component in open-domain QA.
Given a collection of $M$ text passages, the goal of our dense passage retriever (\model/) is to index all the passages in a low-dimensional and continuous space,
such that it can retrieve efficiently the top $k$ passages relevant to the input question for the reader at run-time.
Note that $M$ can be very large
(e.g., 21 \text{million} passages in our experiments, described in Section~\ref{sec:wiki-preprocessing})
and $k$ is usually small, such as $20$--$100$.


\subsection{Overview}
Our dense passage retriever (\model/) uses a dense encoder $E_P(\cdot)$ which maps any text passage to a $d$-dimensional real-valued vectors and builds an index for all the $M$ passages that we will use for retrieval.
At run-time, \model/ applies a different encoder $E_Q(\cdot)$ that maps the input question to a $d$-dimensional vector, and retrieves $k$ passages
of which vectors are the closest to the question vector. We define the similarity between the question and the passage using the dot product of their vectors:
\begin{align}
    \mathrm{sim}(q, p) = E_Q(q)^{\intercal} E_P(p).
    \label{eq:sim}
\end{align}
Although more expressive model forms for measuring the similarity between a question and a passage do exist, such as networks consisting of multiple layers of cross attentions, the similarity function needs to be decomposable so that the representations of the collection of passages can be pre-computed.
Most decomposable similarity functions are some transformations of Euclidean distance (L2). For instance, cosine is equivalent to inner product for unit vectors and the Mahalanobis distance is equivalent to L2 distance in a transformed space.
Inner product search has been widely used and studied, as well as its connection to cosine similarity and L2 distance~\cite{mussmann2016learning,ram2012maximum}.
As our ablation study finds other similarity functions perform comparably (Section~\ref{sec:sim_loss}; Appendix~\ref{sec:alt-sim}), we thus choose the simpler inner product function and improve the dense passage retriever by learning better encoders.

\paragraph{Encoders}
Although in principle the question and passage encoders can be implemented by any neural networks, in this work we use two independent BERT~\cite{devlin2018bert} networks (base, uncased) and take the representation at the \ttt{[CLS]} token as the output, so $d = 768$.

\paragraph{Inference}
During inference time, we apply the passage encoder $E_P$ to all the passages and index them using FAISS \cite{johnson2017billion} offline.
FAISS is an extremely efficient, open-source library for similarity search and clustering of dense vectors, which can easily be applied to billions of vectors.
Given a question $q$ at run-time, we derive its embedding $v_q = E_Q(q)$ and retrieve the top $k$ passages with embeddings closest to $v_q$.


\subsection{Training}\label{sec:training}

Training the encoders so that the dot-product similarity (Eq.~\eqref{eq:sim}) becomes a good ranking function for retrieval is essentially a \emph{metric learning} problem~\cite{kulis2013metric}.
The goal is to create a vector space such that relevant pairs of questions and passages will have smaller distance (i.e., higher similarity) than the irrelevant ones, by learning a better embedding function.

Let $\mathcal{D} = \{ \langle q_i, p^+_i, p^-_{i,1}, \cdots, p^-_{i,n} \rangle \}_{i=1}^m$ be the training data that consists of $m$ instances.
Each instance contains one question $q_i$ and one relevant (positive) passage $p^+_i$, along with $n$ irrelevant (negative) passages $p^-_{i,j}$.
We optimize the loss function as the negative log likelihood of the positive passage:
\begin{eqnarray}
&& L(q_i, p^+_i, p^-_{i,1}, \cdots, p^-_{i,n}) \label{eq:training} \\
&=& -\log \frac{ e^{\mathrm{sim}(q_i, p_i^+)} }{e^{\mathrm{sim}(q_i, p_i^+)} + \sum_{j=1}^n{e^{\mathrm{sim}(q_i, p^-_{i,j})}}}. \nonumber
\end{eqnarray}

\paragraph{Positive and negative passages}
For retrieval problems, it is often the case that positive examples are available explicitly, while negative examples need to be selected from an extremely large pool.
For instance, passages relevant to a question may be given in a QA dataset, or can be found using the answer.
All other passages in the collection, while not specified explicitly, can be viewed as irrelevant by default.
In practice, how to select negative examples is often overlooked but could be decisive for learning a high-quality encoder.
We consider three different types of negatives: (1) Random: any random passage from the corpus; (2) BM25: top passages returned by BM25 which don't contain the answer but match most question tokens; (3) Gold: positive passages paired with other questions which appear in the training set. We will discuss the impact of different types of negative passages and training schemes in Section~\ref{sec:ir_ablation}.
Our best model uses gold passages from the same mini-batch and one BM25 negative passage.
In particular, re-using gold passages from the same batch as negatives can make the computation efficient while achieving great performance.
We discuss this approach below.

\paragraph{In-batch negatives}
Assume that we have $B$ questions in a mini-batch and each one is associated with a relevant passage. Let $\mathbf{Q}$ and $\mathbf{P}$ be the $(B\times d)$ matrix of question and passage embeddings in a batch of size $B$.
$\mathbf{S} = \mathbf{Q}\mathbf{P}^T$ is a $(B\times B)$ matrix of similarity scores, where each row of which corresponds to a question, paired with $B$ passages.
In this way, we reuse computation and effectively train on $B^2$ ($q_i$, $p_j$) question/passage pairs in each batch.
Any ($q_i$, $p_j$) pair is a positive example when $i=j$, and negative otherwise.
This creates $B$ training instances in each batch, where there are $B-1$ negative passages for each question.

The trick of in-batch negatives has been used in the full batch setting~\cite{yih2011learning} and more recently
for mini-batch~\cite{henderson2017efficient,gillick-etal-2019-learning}.
It has been shown to be an effective strategy for learning a dual-encoder model %
that boosts the number of training examples.


==> DPR/sections/sewon-exp-qa.tex <==

\input{tables/sewon-tab-qa.tex}


\section{Experiments: Question Answering}
\label{sec:exp-qa}

In this section, we experiment with how different passage retrievers affect the final QA accuracy.

\subsection{End-to-end QA System}

We implement an end-to-end question answering system in which we can plug different retriever systems directly. 
Besides the retriever, our QA system consists of a neural \textit{reader} that outputs the answer to the question.
Given the top $k$ retrieved passages (up to $100$ in our experiments), the reader assigns a passage selection score to each passage.  
In addition, it extracts an answer span from each passage and assigns a span score.
The best span from the passage with the highest passage selection score is chosen as the final answer.
The passage selection model serves as a reranker through cross-attention between the question and the passage. 
Although cross-attention is not feasible for retrieving relevant passages in a large corpus due to its non-decomposable nature, it has more capacity than the dual-encoder model $\mathrm{sim}(q,p)$ as in Eq.~\eqref{eq:sim}. Applying it to selecting the passage from a small number of retrieved candidates has been shown to work well~\cite{wang2019multi, wang2018r, lin2018denoising}.

Specifically, let $\mathbf{P}_{i} \in \mathbb{R}^{L \times h}$ ($1 \leq i \leq k$) be a BERT (base, uncased in our experiments) representation for the $i$-th passage, where $L$ is the maximum length of the passage and $h$ the hidden dimension.
The probabilities of a token being the starting/ending positions of an answer span and a passage being selected are defined as:
\begin{eqnarray}
    P_{\textrm{start},i}(s)  &=& \mathrm{softmax} \big( \mathbf{P}_{i} \mf{w}_\textrm{start}\big)_s, \\
    P_{\textrm{end},i}(t) &=& \mathrm{softmax} \big( \mathbf{P}_{i} \mf{w}_\textrm{end}\big)_t, \\
    P_\textrm{selected}(i) &=& \mathrm{softmax} \big( \mathbf{\hat{P}}^{\intercal} \mf{w}_\mathrm{selected}  \big)_i,
\end{eqnarray} where $\mathbf{\hat{P}} = [\mathbf{P}_1^{\mathrm{[CLS]}}, \ldots, \mathbf{P}_k^{\mathrm{[CLS]}}] \in \mathbb{R}^{h \times k}$ and $\mf{w}_\textrm{start}, \mf{w}_\textrm{end},\mf{w}_\mathrm{selected} \in \mathbb{R}^{h}$ are learnable vectors. 
We compute a span score of the $s$-th to $t$-th words from the $i$-th passage as $P_{\textrm{start},i}(s) \times P_{\textrm{end},i}(t)$, and a passage selection score of the $i$-th passage as $P_\textrm{selected}(i)$.

During training, we sample one positive and $\tilde{m}-1$ negative passages from the top 100 passages returned by the retrieval system (BM25 or DPR) for each question.  $\tilde{m}$ is a hyper-parameter and we use $\tilde{m}=24$ in all the experiments. The training objective is to maximize the marginal log-likelihood of all the correct answer spans in the positive passage (the answer string may appear multiple times in one passage), combined with the log-likelihood of the positive passage being selected. We use the batch size of 16 for large (NQ, TriviaQA, SQuAD) and 4 for small (TREC, WQ) datasets, and tune $k$ on the development set. For experiments on small datasets under the {\em Multi} setting, in which using other datasets is allowed, we fine-tune the reader trained on Natural Questions to the target dataset. All experiments were done on eight 32GB GPUs.




\subsection{Results}

Table~\ref{tab:qa_em} summarizes our final end-to-end QA results, measured by \emph{exact match} with the reference answer after minor normalization as  in~\cite{chen2017reading,lee2019latent}.  From the table, we can see that higher retriever accuracy typically leads to better final QA results: 
in all cases except SQuAD, answers extracted from the passages retrieved by \model/ are more likely to be correct, compared to those from BM25.
For large datasets like NQ and TriviaQA, models trained using multiple datasets (Multi) perform comparably to those trained using the individual training set (Single).  Conversely, on smaller datasets like WQ and TREC, the multi-dataset setting has a clear advantage. Overall, our \model/-based models outperform the previous state-of-the-art results on four out of the five datasets, with 1\% to 12\% absolute differences in exact match accuracy.
It is interesting to contrast our results to those of ORQA~\cite{lee2019latent} and also the concurrently developed approach, REALM~\cite{guu2020realm}. While both methods include additional pretraining tasks and employ an expensive end-to-end training regime, \model/ manages to outperform them on both NQ and TriviaQA, simply by focusing on learning a strong passage retrieval model using pairs of questions and answers.
The additional pretraining tasks are likely more useful only when the target training sets are small. Although the results of \model/ on WQ and TREC in the single-dataset setting are less competitive, adding more question--answer pairs helps boost the performance, achieving the new state of the art.

To compare our pipeline training approach with joint learning, we run an ablation on Natural Questions where the retriever and reader are jointly trained, following \citet{lee2019latent}.
This approach obtains a score of 39.8 EM, which suggests that our strategy of training a strong retriever and reader in isolation can leverage effectively available supervision, while outperforming a comparable joint training approach with a simpler design (Appendix~\ref{sec:joint}).

One thing worth noticing is that our reader does consider more passages compared to ORQA, although it is not completely clear how much more time it takes for inference. 
While \model/ processes up to 100 passages for each question, the reader is able to fit all of them into one batch on a single 32GB GPU, thus the latency remains almost identical to the single passage case (around 20ms).
The exact impact on throughput is harder to measure: ORQA uses 2-3x longer passages compared to DPR (288 word pieces compared to our 100 tokens) and the computational complexity is super-linear in passage length. We also note that we found $k=50$ to be optimal for NQ, and $k=10$ leads to only marginal loss in exact match accuracy (40.8 vs. 41.5 EM on NQ), which should be roughly comparable to ORQA's 5-passage setup.






==> DPR/tables/ir-ablation.tex <==

\begin{table}[t]
    \centering
    \small
    \begingroup
    \setlength{\tabcolsep}{0.70\tabcolsep}
    \begin{tabular}{@{}l l c cc c c @{}} \toprule
    \tf{Type} & \tf{\#N} & \tf{IB} & \tf{Top-5} & \tf{Top-20} & \tf{Top-100} \\ \midrule
    Random & 7 & $\xmark$ & 47.0 & 64.3 & 77.8 \\
    BM25 & 7 & $\xmark$ & 50.0 & 63.3 & 74.8\\
    Gold & 7 & $\xmark$ & 42.6 & 63.1 & 78.3\\
    \midrule
    Gold & 7 & $\cmark$ & 51.1 & 69.1 & 80.8 \\
    Gold & 31 & $\cmark$ & 52.1 & 70.8 & 82.1 \\
    Gold & 127 & $\cmark$ & 55.8 & 73.0 & 83.1\\
    \midrule
    G.+BM25$^{(1)}$ & 31+32 & $\cmark$ & 65.0 & 77.3 & 84.4 \\
    {G.+BM25}$^{(2)}$ & 31+64 & $\cmark$ & 64.5 & 76.4 & 84.0 \\
    G.+BM25$^{(1)}$ & 127+128 & $\cmark$ & \tf{65.8} & \tf{78.0} & \tf{84.9} \\
    \bottomrule
    \end{tabular}
    \endgroup
    \caption{Comparison of different training schemes, measured as top-$k$ retrieval accuracy on Natural Questions (development set).  \#N: number of negative examples, IB: in-batch training. G.+BM25$^{(1)}$ and {G.+BM25}$^{(2)}$ denote in-batch training with 1 or 2 additional BM25 negatives, which serve as negative passages for all questions in the batch.} 
    
    


    \label{tab:ir-ablation}
\end{table}


==> DPR/tables/qa_ir_dist_sv.tex <==

\begin{table}[t!]
    \setlength\tabcolsep{5pt}
    \centering
    \begin{tabular}{lcccc} \toprule
         & \tf{Top-1} & \tf{Top-5} & \tf{Top-20} & \tf{Top-100}  \\ \midrule
        {Gold} & 44.9 & 66.8 & 78.1 & 85.0 \\
        {Dist. Sup.} & 43.9 & 65.3 & 77.1 & 84.4 \\
    \bottomrule
    \end{tabular}
    \caption{
    Retrieval accuracy on the development set of Natural Questions, trained on passages that match the gold context (Gold) or the top BM25 passage that contains the answer (Dist. Sup.).
    }
    \label{tab:qa_ir_dist_sv}
\end{table}



==> DPR/tables/qa_ir_sim_and_loss.tex <==
\begin{table}[t!]
    \setlength\tabcolsep{4pt}
    \centering
    \begin{tabular}{ll|cccc}
    \toprule
    \tf{Sim} & \tf{Loss} & \multicolumn{4}{c}{\tf{Retrieval Accuracy}} \\ 
    & & Top-1 & Top-5 & Top-20 & Top-100 \\ \midrule
    \multirow{2}{*}{DP} & NLL & \tf{44.9} & \tf{66.8} & \tf{78.1} & \tf{85.0} \\
    & Triplet & 41.6 & 65.0 & 77.2 & 84.5 \\
    \midrule
    \multirow{2}{*}{L2} & NLL & 43.5 & 64.7 & 76.1 & 83.1 \\
    & Triplet & 42.2 & 66.0 & \tf{78.1} & 84.9 \\ 
    \bottomrule
    \end{tabular}
     \caption{Retrieval Top-$k$ accuracy on the development set of Natural Questions using different similarity and loss functions.} 

    \label{tab:qa_ir_sim_and_loss}
\end{table}
\setlength{\tabcolsep}{6pt} %


==> DPR/tables/retrieval-accuracy.tex <==

\ignore{
\begin{table*}[!ht]
    \centering
    \begin{tabular}{llcccc} \toprule
    $k$ & Retriever & {Natural Questions} & {TriviaQA} & {WebQuestions} & {CuratedTREC} \\
    \midrule
    \multirow{2}{*}{5} &
    BM25   & 41.6 & 54.4 & 36.8 & 54.9  \\
    & Dense  & \tf{67.0} & \tf{69.7} & \tf{63.9} & \tf{79.9}  \\
    & Dense+ & & & & \\
    \midrule
    \multirow{2}{*}{20} &
        BM25   & 57.9 & 66.9 & 55.0 & 70.9  \\
    & Dense  & \tf{79.4} & \tf{78.8} & \tf{75.0} & \tf{89.1}  \\
    & Dense+ & & & & \\
    \midrule
    \multirow{2}{*}{50} &
        BM25   & 67.7 & 72.8 & 64.5 & 80.3  \\
    & Dense  & \tf{83.8} & \tf{82.5} & \tf{80.5} & \tf{92.6}  \\
    & Dense+ & & & & \\
    \midrule
    \multirow{2}{*}{100} &
        BM25   & 73.2 & 76.7 & 71.1 & 84.1 \\
    & Dense  & \tf{86.0} & \tf{84.7} & \tf{82.9} & \tf{93.9}  \\
    & Dense+ & & & & \\
    \bottomrule
    \end{tabular}
    \caption{Top-$K$ retrieval accuracy, measured as the percentage that top $k$ retrieved passages that contain an answer. The numbers are reported on the testing set.}
    \label{tab:qa_ir}
\end{table*}

}




\begin{table*}[t!]
    \setlength\tabcolsep{5pt}
    \centering
    \small
    \begin{tabular}{ll|ccccc|ccccc}
    \toprule
    \tf{Training} & \tf{Retriever} & \multicolumn{5}{c}{\tf{Top-20}} & \multicolumn{5}{|c}{\tf{Top-100}} \\
    & & NQ & TriviaQA & WQ & TREC & SQuAD & NQ & TriviaQA & WQ & TREC & SQuAD \\ \midrule
    None & BM25 & 59.1 & 66.9 & 55.0 & 70.9 & 68.8 & 73.7 & 76.7 & 71.1 & 84.1 & 80.0 \\
    \midrule
    \multirow{2}{*}{Single} &\model/ & 78.4 & 79.4 & 73.2 & 79.8 & 63.2 & 85.4 & \textbf{85.0} & 81.4 & 89.1 & 77.2 \\
    &BM25 + \model/ & 76.6 & 79.8 & 71.0 & 85.2 & \textbf{71.5} & 83.8 & 84.5 & 80.5 & 92.7 & \textbf{81.3} \\
    \midrule
    \multirow{2}{*}{Multi} &\model/ & \textbf{79.4} & 78.8 & \textbf{75.0} & \textbf{89.1} & 51.6 & \textbf{86.0} & 84.7 & \textbf{82.9} & 93.9 & 67.6 \\
    &BM25 + \model/ & 78.0 & \textbf{79.9} & 74.7 & 88.5 & 66.2 & 83.9 & 84.4 & 82.3 & \textbf{94.1} & 78.6 \\ \bottomrule
    \end{tabular}
     \caption{Top-20 \& Top-100 retrieval accuracy on test sets, measured as the percentage of top 20/100 retrieved passages that contain the answer. \ti{Single} and \ti{Multi} denote that our Dense Passage Retriever (DPR) was trained using individial or combined training datasets (all the datasets excluding SQuAD). See text for more details.} %

    \label{tab:qa_ir}
\end{table*}




==> DPR/tables/retrieved-examples.tex <==
\begin{table*}[!t]
\scriptsize
\begin{tabular}{p{3cm}|p{6cm}|p{6cm}}
\toprule
\tf{Question} & \tf{Passage received by BM25} & \tf{Passage retrieved by \model/} \\
\midrule
\multirow{2}{3cm}{What is the body of water between England and Ireland?} & Title:British Cycling  & Title: Irish Sea\\
& \ldots  \tf{England} is not recognised as a region by the UCI, and there is no English cycling team outside the Commonwealth Games. For those occasions, British Cycling selects and supports the \tf{England} team. Cycling is represented on the Isle of Man by the Isle of Man Cycling Association.  Cycling in Northern \tf{Ireland} is organised under Cycling Ulster, part of the all-Ireland governing \tf{body} Cycling \tf{Ireland}. Until 2006, a rival governing \tf{body} existed,  \ldots & \ldots Annual traffic between Great Britain and \tf{Ireland} amounts to over 12 million passengers and of traded goods. {\color{blue}\tf{The Irish Sea}} is connected to the North Atlantic at both its northern and southern ends. To the north, the connection is through the North Channel between Scotland and Northern \tf{Ireland} and the Malin Sea. The southern end is linked to the Atlantic through the St George's Channel between Ireland and Pembrokeshire, and the Celtic Sea. \ldots \\
\midrule
\multirow{2}{3cm}{Who plays Thoros of Myr in Game of Thrones?} & Title: No One (Game of Thrones) & Title:
P\r{a}l Sverre Hagen \\ & \ldots He may be "no one," but there's still enough of a person left in him to respect, and admire who this girl is and what she's become. Arya finally tells us something that we've kind of known all along, that she's not no one, she's Arya Stark of Winterfell." "No One" saw the reintroduction of Richard Dormer and {\color{blue}\tf{Paul Kaye}}, who portrayed Beric Dondarrion and \tf{Thoros} of \tf{Myr}, respectively, in the third season, \ldots &
P\r{a}l Sverre Valheim Hagen (born 6 November 1980) is a Norwegian stage and screen actor. He appeared in the Norwegian film "Max Manus" and played Thor Heyerdahl in the Oscar-nominated 2012 film "Kon-Tiki". Pål Hagen was born in Stavanger, Norway, the son of Roar Hagen, a Norwegian cartoonist who has long been associated with Norway\'s largest daily, "VG". He lived in Jåtten, a neighborhood in the city of Stavanger in south-western Norway. \ldots \\
\bottomrule
\end{tabular}
\caption{Examples of passages returned from BM25 and \model/. Correct answers are written in {\color{blue} \tf{blue}} and the content words in the question are written in bold.}
\label{tab:retrieved-examples}
\end{table*}



==> DPR/tables/sewon-tab-qa.tex <==
\newcommand{\nqbm}{32.6}
\newcommand{\nqsingle}{\tf{41.5}}
\newcommand{\nqsinglehybrid}{39.0}
\newcommand{\nqmulti}{\tf{41.5}}
\newcommand{\nqmultihybrid}{38.8}

\newcommand{\triviabm}{52.4}
\newcommand{\triviasingle}{56.8}
\newcommand{\triviasinglehybrid}{57.0}
\newcommand{\triviamulti}{56.8}
\newcommand{\triviamultihybrid}{\tf{57.9}}

\newcommand{\sqbm}{38.1}
\newcommand{\sqsingle}{29.8}
\newcommand{\sqsinglehybrid}{36.7}
\newcommand{\sqmulti}{24.1}
\newcommand{\sqmultihybrid}{35.8}

\newcommand{\webqbm}{29.9}
\newcommand{\webqsingle}{34.6}
\newcommand{\webqsinglehybrid}{35.2}
\newcommand{\webqmulti}{\tf{42.4}}
\newcommand{\webqmultihybrid}{41.1}

\newcommand{\trecbm}{24.9}
\newcommand{\trecsingle}{25.9}
\newcommand{\trecsinglehybrid}{28.0}
\newcommand{\trecmulti}{49.4}
\newcommand{\trecmultihybrid}{\tf{50.6}}

\begin{table*}[t]
    \setlength\tabcolsep{5pt}
    \centering
    \begin{tabular}{llccccc} \toprule
    \tf{Training} & \tf{Model} & \tf{NQ} & \tf{TriviaQA} & \tf{WQ} & \tf{TREC} & \tf{SQuAD} \\ \midrule
    Single & {BM25+BERT}~\cite{lee2019latent} & 26.5 & 47.1 & 17.7 & 21.3 & 33.2 \\
    Single & {ORQA}~\cite{lee2019latent}  & 33.3 & 45.0 & 36.4 & 30.1 & 20.2   \\
    Single & {HardEM}~\cite{min2019discrete} & 28.1 & 50.9 & - & - & - \\
    Single & {GraphRetriever}~\cite{min2019knowledge} & 34.5 & 56.0 & 36.4 & - & - \\
    Single & {PathRetriever}~\cite{asai2020learning}  & 32.6 & - & - & - & \tf{56.5}\\
    Single & {REALM}$_\textrm{Wiki}$~\cite{guu2020realm} & 39.2 & - & 40.2 & 46.8 & - \\ 
    Single & {REALM}$_\textrm{News}$~\cite{guu2020realm} & 40.4 & - & 40.7 & 42.9 & - \\ 
    \midrule
    \multirow{3}{*}{Single} & BM25   & \nqbm & \triviabm & \webqbm & \trecbm & \sqbm \\
    &\model/  & \nqsingle & \triviasingle & \webqsingle & \trecsingle & \sqsingle \\
    &BM25+\model/  & \nqsinglehybrid & \triviasinglehybrid & \webqsinglehybrid & \trecsinglehybrid & \sqsinglehybrid \\
    \midrule
    \multirow{2}{*}{Multi} & \model/  & \nqmulti & \triviamulti & \webqmulti & \trecmulti & \sqmulti \\
    &BM25+\model/ & \nqmultihybrid & \triviamultihybrid & \webqmultihybrid & \trecmultihybrid & \sqmultihybrid \\
    \bottomrule
    \end{tabular}
    \caption{End-to-end QA (Exact Match) Accuracy. The first block of results are copied from their cited papers. {REALM}$_\textrm{Wiki}$ and {REALM}$_\textrm{News}$ are the same model but pretrained on Wikipedia and CC-News, respectively.
    \ti{Single} and \ti{Multi} denote that our Dense Passage Retriever (DPR) is trained using individual or combined training datasets (all except SQuAD). For WQ and TREC in the \ti{Multi} setting, we fine-tune the reader trained on NQ.}
    \label{tab:qa_em}
\end{table*}


==> DPR/tables/split-stats.tex <==
\begin{table}[!t]
    \small
    \centering
    \begin{tabular}{lrrrr} \toprule
    \tf{Dataset} & \multicolumn{2}{c}{\tf{Train}}  & \tf{Dev} & \tf{Test} \\
    \midrule
    Natural Questions   & 79,168 & 58,880 & 8,757 & 3,610 \\
    TriviaQA            & 78,785 & 60,413 & 8,837 & 11,313  \\
    WebQuestions        & 3,417  & 2,474 & 361   & 2,032 \\
    CuratedTREC         & 1,353  & 1,125 & 133   & 694 \\
    SQuAD               & 78,713 & 70,096 & 8,886 & 10,570  \\
    \bottomrule
    \end{tabular}
    \caption{Number of questions in each QA dataset. The two columns of \textbf{Train} denote the original training examples in the dataset and the actual questions used for training DPR after filtering.  See text for more details.}
    \label{tab:split-stats}
\end{table}



==> proposal.tex <==
% Title: Dense Passage Retrieval in Conversational Search

% Description: One of the recognized problems in Information Retrieval (IR) is the conversational search that attracts much attention in form of Conversational Assistants such as Alexa, Siri and Cortana. The users’ needs are the ultimate goal of conversational search systems, in this context the questions are asked sequentially imposing a multi-turn format as the Conversational Information Seeking (CIS) task. TREC Conversational Assistance Track (CAsT) [3] is a multi-turn conversational search task as it contains a large-scale reusable test collection for sequences of conversational queries. The response of this conversational model is not a list of relevant documents, but it is limited to brief response passages with a length of 1 to 3 sentences in length.

% Example Queries in CAsT

% In [4], the authors focus on improving open domain question answering by including dense representations for retrieval instead of the traditional methods. They have adopted a simple dual-encoder framework to construct a learnable retriever on large collections. We want to adopt this dense representation for the conversational model in the CAsT task and compare it with the performance of the other approaches in literature. The performance will be indicated by using graded relevance on five point, which are Fails to meet, Slightly meets, Moderately meets, Highly meets, and Fully meets.

% We aim to further improve our system performance by integrating the following techniques:

% • Paragraph-level pre-training tasks: ICT, BFS, and WLP [1]

% • ANCE training: periodically using checkpoints to encode documents, from which the strong negatives close to the relevant document would be used as next training negatives [5]

% In summary, this project is exploratory in nature as we will be trying to use state-of-art Dense Passage Retrieval techniques (based on BERT) [4, 6], in a question answering (QA) problem. Current first-stage-retrieval approaches mainly rely on bag-of-words models. In this project, we hope to explore the feasibility of using state-of-art methods such as BERT. We will first compare how these perform on the TREC CAsT datasets [3] against the results retrieved using BM25. After these first points of comparison we will next explore methods of improving DPR by exploring one or more techniques that are made to improve the performance of DPR. [1, 5].

% References

% [1] Wei-Cheng Chang et al. Pre-training Tasks for Embedding-based Large-scale Retrieval. 2020. arXiv: 2002.03932 [cs.LG].

% [2] Zhuyun Dai and Jamie Callan. Context-Aware Sentence/Passage Term Importance Estimation For First Stage Retrieval. 2019. arXiv: 1910.10687 [cs.IR].

% [3] Jeffrey Dalton, Chenyan Xiong, and Jamie Callan. TREC CAsT 2019: The Conversational Assistance Track Overview. 2020. arXiv: 2003.13624 [cs.IR].

% [4] Vladimir Karpukhin et al. Dense Passage Retrieval for Open-Domain Ques- tion Answering. 2020. arXiv: 2004.04906 [cs.CL].

% [5] Lee Xiong et al. Approximate Nearest Neighbor Negative Contrastive Learn- ing for Dense Text Retrieval. 2020. arXiv: 2007.00808 [cs.IR].

% [6] Jingtao Zhan et al. RepBERT: Contextualized Text Embeddings for First- Stage Retrieval. 2020. arXiv: 2006.15498 [cs.IR].
